Adaptive Algorithms for Relaxed Pareto Set Identification

In this paper we revisit the fixed-confidence identification of the Pareto optimal set in a multi-objective multi-armed bandit model. As the sample complexity to identify the exact Pareto set can be very large, a relaxation allowing to output some additional near-optimal arms has been studied. In this work we also tackle alternative relaxations that allow instead to identify a relevant subset of the Pareto set. Notably, we propose a single sampling strategy, called Adaptive Pareto Exploration, that can be used in conjunction with different stopping rules to take into account different relaxations of the Pareto Set Identification problem. We analyze the sample complexity of these different combinations, quantifying in particular the reduction in sample complexity that occurs when one seeks to identify at most $k$ Pareto optimal arms. We showcase the good practical performance of Adaptive Pareto Exploration on a real-world scenario, in which we adaptively explore several vaccination strategies against Covid-19 in order to find the optimal ones when multiple immunogenicity criteria are taken into account.

==> parts/appx-archive.tex <==
%\section{Outline}
\section{Outline and Notation}
In this section, we provide an outline of the supplemental material and define some additional notation. In \autoref{sec:proof_thm1}, we prove \autoref{thm:sampcompl} and the lemmas used in its proof. 
%TODO 
In \autoref{sec:alg_eps_2} we show to modify the stopping rule of \algname to get a $(\eps_1, \eps_2,m,\delta)-$PAC algorithm. In \autoref{sec:tech_lemmas} we recall or prove some technical lemmas that are used in the main proofs. In \autoref{sec:impl_exp} we give further details about the experiments together with additional experimental results. 
\begin{table}[ht]
    \centering
    \begin{tabular}{p{2cm}p{3cm}p{7cm}}
    \hline 
         Notation&Type&Description  \\
         \hline 
         $\bA$ & & Set of arms\\
         $K$ & $\bN^\star$ & Number of arms \\
         $D$ & $\bN^\star$ & Dimension or number of attributes \\ 
         $[n]$ & & $\{1,\dots, n\}$\\ 
         $\m$ & $\bA^2 \rightarrow \bR$ & $\m(i,j) := \min\{ \mu_j^d - \mu_i^d: d\in [D] \}$\\
         $\M$ & $\bA^2 \rightarrow \bR$ & $\M(i,j) := \max\{ \mu_i^d - \mu_j^d: d\in [D] \}$ \\
         $(x)^+$ & $\bR\rightarrow \bR^+$ &$ \max(0, x)$ \\
         $\vmu_a$ & $\bR^D$ & Mean of arm $a \in \bA$ \\
         $\cS^\star_{\eps}$  & & $\{i \in \bA: \nexists j\neq i \in \bA : \vmu_i + \eps \prec \vmu_j \}$\\
         $\Delta_a^{(m, \eps)}$ & $\bR$ & $\max(\Delta_a, \eps, \omega^{(m)})$\\
         $H_{m,\eps_1}$ & $\bR$ & $\sum_{k=1}^K (\Delta_k^{(\eps, m)})^{-2}$ \\
         \hline 
         
    \end{tabular}
    \caption{Table of notation.}
    \label{tab:notation}
\end{table}
\section{Proof of \autoref{thm:sampcompl}}
\label{sec:proof_thm1}
In this section we prove \autoref{thm:sampcompl} which is restated below. 
\mainTheorem
We state the following lemma which will be used to derive an upper bound on the gap of an optimal arm. Moreover it shows that for sub-optimal arms, the $\max$ operator appearing in the definition of the gap can be extending to the whole $\bA$ instead of $\cS^\star$ which gives an easy way to empirically estimate this quantity.  
\begin{lemma} 
\label{lem:existence_dom}
For any sub-optimal arm $a$, there exists a Pareto optimal arm $a^\star$ such that $\vmu_a \prec \vmu_{a^\star}$ and $\Delta_{a} = \m(a, a^\star)$. Moreover, For any $i\in \bA\setminus \cS^\star$, $j \in \cS^\star$, 
\begin{enumerate}[i)]
    \item $\max_{k\in \cS^\star} \m(i,k) = \max_{k\in \bA} \m(i,k)$, 
    \item If $i \in \argmin_{k\in \bA \setminus \{j\}} \M(j,k)$ then $j$ is the unique arm such that $\vmu_i \prec \vmu_j$ 
\end{enumerate}
\begin{proof}
Suppose that there are $k<n$ dominated vectors in $\cS^\star.$ Without loss of generality, we may assume they are $\vmu_1, \dots, \vmu_k$. Let $i_1\leq k$. Suppose that no Pareto-optimal vector dominates $\vmu_{i_1}$. Since $\vmu_{i_1}$ is not optimal, by the latter assumption, there exists $i_2 \leq k$ such that $\vmu_{i_1}\prec \vmu_{i_2}$. If $\vmu_{i_2}$ is dominated by a Pareto optimal vector, this vector also dominates $\vmu_{i_1}$ (by transitivity) which contradicts the initial assumption. If not, there exits $i_3 \leq k$ such that $\vmu_{i_1}\preceq \vmu_{i_2}\preceq \vmu_{i_3}$. Again we can use the same reasoning as before for $i_3$. In any case we should stop in at most $k$ steps, otherwise we would have $\vmu_{i_1}\prec \vmu_{i_2}\prec \dots \prec \vmu_{i_k}$ and $\vmu_{i_k}$ should be dominated by a Pareto-optimal vector, otherwise it would be itself Pareto-optimal, which is not the case. Therefore, for any $a\in \bA\setminus \cS^\star$, there exists $a^\star \in \cS^\star$ such that $a^\star \prec a, \tm{ and } \Delta_a = \m(a, a^\star)>0$. Moreover, for any $k\in \bA\setminus \cS^\star$, since $a\prec a^\star$, 
\[ \forall  d \in [D],\; \mu_a^d - \mu_k^d \leq \mu_{a^\star}^d - \mu_k^d,\]
which leads to $\m(k, a) \leq \m(k, a^\star)$, so 
\[  \max_{j\in \bA} \m(i,j) = \max_{j\in \cS^\star} \m(i,j),\]
which proves the first point {\it i)}. For the second point, let $k \in \bA\setminus \cS^\star$ and $k'\neq k$ such that $k\prec k'$ and \[ k \in \argmin_{l\in \bA \setminus \{j\}} \M(j,l).\] By direct algebra, since $k\prec k'$, we would have 
\[ \M(j, k') < \M(j, k),\] which is impossible, if there exists $k'\neq j$. 
\end{proof}
\end{lemma}
Then the next lemma follows directly from this result. 
\begin{lemma}
\label{lem:gap_opt}
    For any Pareto optimal arm $i$, $\Delta_i \leq \min_{j\neq i} \M(i,j).$
\end{lemma}
\begin{proof}
If $\argmin_{j\neq i} \M(i,j) \subset \cS^\star$, then the lemma follows from the definition of the gap of an optimal arm. If $\min_{j\neq i} \M(i,j) = \M(i, a)$, $a\notin \cS^\star$, then, 
    from \autoref{lem:existence_dom}, $i$ is the unique arm which dominates $a$ so $\Delta_a = \m(a, i)$ and using the definition of the gap of an optimal arm, \begin{eqnarray*}
        \Delta_i &\leq& \M(a, i)^+ + \Delta_a, \\
        &=& 0 + \m(a, i) \leq \M(i,a),
    \end{eqnarray*}
    where we have used the the fact that (which follows from the definition) $\m(p,q)\leq \M(q, p)$ for any pair of arms $p,q$. Therefore, we always have 
    $$ \Delta_i \leq \min_{j\neq i} \M(i,j).$$
\end{proof}

\begin{lemma}
\label{lem:stoppingcond}
    During round $t$, if $Z_1^{\eps_1}(t) \leq 0 $ or $Z_2^{\eps
_1}(t) \leq 0$ then for any $j\in \bA$, $\mh(b_t,j,t)\leq \beta_{b_t, j}(t).$
    \end{lemma}

    \begin{proof}
    Assume there exits $j$ such that $\mh(b_t,j,t) > \beta_{b_t, j}(t)$. Equivalently, we have $\Mh(b_t, j, t) +  \beta_{b_t ,t}(t) <0 $. So from the definition of $b_t$, for any $i \in \OPT^{\eps_1}(t)^\complement$, there exists an arm $k$ such that $$\Mh(i, k, t)  + \beta_{i, k}(t) <0, $$ i.e. $\mh(i,k,t)>\beta_{i, k}(t)$. In particular such an arm $i$ satisfies $\max_{k} \mh(i,k,t)> 0$ and belongs to $S(t)^\complement$. It comes that $\OPT^{\eps_1}(t)^\complement \subset S(t)^\complement$ that is $$S(t) \subset \OPT^{\eps_1}(t),$$ so $Z_1^{\eps_1}(t) >0$. On the other side, for any $i \in \OPT^{\eps_1}(t) \cap S(t)$, $h^{\eps_1}_i(t) >0$ therefore,  $Z_2^{\eps_1}(t)>0$. Putting things together, if the initial assumption holds, then $Z^{\eps_1}_1(t) > 0$ and $Z^{\eps_1}_2(t)> 0$. 
    \end{proof}

%         \begin{proof}
%     Assume there exits $j$ such that $\m(b_t,j,t) > \beta_j(t) + \beta_{b_t}(t)$, then for any $d\in \{1, \dots, D\}$, $\muh_{b_t}^d(t) + \beta_{b_t}(t) < \muh_j^d(t) - \beta_j(t)$. Which yields $\M(b_t, j, t)  + \beta_{b_t}(t) + \beta_j(t) <0 $. So, for any $i \in \tm{OPT}_t^\mathsf{c}$, there exists an arm $k$ such that $\M(i, k, t)  + \beta_{i}(t) + \beta_k(t) <0 $, which yields, $$\max_{d}(\muh_i^d(t) - \muh_k^d(t)) < -\beta_{i}(t) - \beta_k(t), $$
% then $\m(i,k,t)>\beta_{i}(t) + \beta_k(t)$. Noting that such an arm $i$ belongs to $\cS(t)^\mathsf{c}$, it comes that $\tm{OPT}_t^\mathsf{c} \subset \cS(t)^\mathsf{c}$. On the other side, letting $i\in \tm{OPT}_t$, for any $j\neq i$, there exists $d$ such that $\muh_i^d(t) - \beta_i(t) > \muh_j^d(t) + \beta_j(t)$ thus $\vmu_i(t) \nprec \vmu_j(t)$ so $i\in \cS(t)$. Putting things together lead to : $\tm{OPT}_t = \cS(t)$ so $\tm{OPT}_t^\mathsf{c} = \cS(t)^\mathsf{c}$ and for any $i\in \cS(t)^\mathsf{c}$ there exists $j\neq i$ such that $\m(i,j,t)> \beta_i(t) + \beta_j(t)$. Which yields $Z_1(t) > 0$ and $Z_2(t)> 0$. 
%     \end{proof}
    
 %  \todoe{J'ai réécrit un peu la preuve en la simplifiant en utilisant $M=-m$, vois si ça te va. La version précédente est commentée.} 
    
%    \medskip
%    \textcolor{red}{Tu as l'air d'utiliser à trois reprises dans les preuves des lemmes ci-dessous que lorsque $(Z_1(t) \leq 0)$ ou $(Z_2(t) \leq 0)$ on a $M(b_t,c_t,t) - \beta_{b_t}(t) - \beta_{c_t}(t) < 0$ (j'ai mis en rouge toutes les inégalités qui me semblent utiliser cela). Est-ce que c'est vrai ? Ou peut être que je n'ai pas compris et que tu utilises autre chose.}
%maybe inutile 
%\begin{lemma}
%\label{lem:smplemmadom}
%For any round $t$, if the event $\cE_t$ holds then for any sub-optimal arm $a$, if $a^\star \notin U^a_t$ then $\Delta_a \leq 2\beta_a(t)$. 
 %\begin{proof}
 %    Assume $\cE_t$ holds. Let $a \notin \cS^\star$. We know from  \autoref{lem:existence_dom}, that there always exists $a^\star \in \cS^\star$ such that $a\prec a^\star$ and $\Delta_a = \m(a, a^\star)$. We have 
 %    \begin{eqnarray}
 %        a^\star \notin U^a_t &\impl& \exists d \in [D] \; \tm{ s.t } \;\muh_a(t) + \beta_a(t) \geq \muh_{a^\star}(t) + \beta_{a^\star}(t) \overset{\cE_t}{\geq}\mu_{a^\star}^d\\
 %        &\impl& \exists d \in [D] \; \tm{ s.t } \;
 %        \mu_a^d + 2\beta_a(t) \overset{\cE_t}{\geq} \muh_a(t) - \beta_a(t) + 2\beta_a(t) \geq  \mu_{a^\star}^d\\
 %         &\impl& \exists d \in [D] \; \tm{ s.t } \;
 %        \mu_{a^\star}^d - \mu_{a}^d \leq 2\beta_a(t) \\
 %        &\impl& \Delta_a := \min_{d} (\mu_{a^\star}^d - \mu_{a}^d) \leq 2\beta_a(t). 
 %    \end{eqnarray}
 %\end{proof}
%\end{lemma} 
%\todoe{proof?}
\subsection{Proof of Lemma~\ref{lem:samplwm}}
Assume $\cE_t$ holds. Let $k\leq\lvert\cS^\star\lvert$. If $t < \tau_{\delta}^{\eps_1, m}$ then it holds that $\lvert\OPT^{\eps_1}(t)\lvert < k$. That is $\cS^{\star, k} \cap {\OPT^{\eps_1}(t)}^\complement \neq \emptyset$. Let $i\in\cS^{\star, k} \cap {\OPT^{\eps_1}(t)}^\complement$, we have 
\begin{eqnarray*}
    \omega^k &\leq& \omega_i = \min_{j \in \bA \setminus\{i\}} \M(i,j),\\
    &\overset{(a)}{\leq}& \min_{j \in \bA \setminus\{i\}} \M(i,j, t) + \beta_{i,j}(t), \\
    &\overset{(b)}{\leq}& \min_{j \in \bA \setminus\{b_t\}} \Mh(b_t,j, t) + \beta_{b_t, j}(t),\\
    &\leq& \Mh(b_t,c_t, t) + \beta_{b_t, c_t}(t) ,\\
    &{\overset{(c)}{\leq}}& \ 2\beta_{b_t, c_t}(t), %+ \beta_{c_t}(t)) \leq 4\beta_{k_t}(t),
\end{eqnarray*}
where $(a)$ uses that $\cE_t$ holds, $(b)$ uses the definition of $b_t$ and $(c)$ follows from the definition of $c_t$ and the fact that $b_t \notin \OPT^{\eps
_1}(t)$. 
%\todoe{TODO: Corriger les ``autoref'' qui pointent sur des théorèmes plutôt que des lemmes}
\subsection{Proof of \autoref{lem:ineq_gene}}
\begin{proof}
Assume $\cE_t$ holds. We have 
    \begin{eqnarray*}
        \lvert \M(i,j) - \Mh(i,j,t)\lvert &=& \lvert \max_d (\muh_i^d(t) - \muh_j^d(t))- \max_d (\mu_i^d - \mu_j^d)\lvert, \\ &\overset{(a)}{\leq}& \max_d \lvert (\muh_i^d(t)  - \muh_j^d(t)) -  (\mu_i^d - \mu_j^d)\lvert,  \\%\stepcounter{equation}\tag{\theequation} \label{eq:lemIneqL1}, 
        %\\&=& \max_d \lvert (\muh_i^d(t)  - \mu_i^d) -  (\muh_j^d(t) - \mu_j^d)\lvert, \\&\leq& \lVert \vmuh_i(t)  - \vmu_i \lVert_\infty + \lVert \vmuh_j(t)  - \vmu_j \lVert_\infty, \\ 
        &\overset{(b)}{\leq}& \beta_{i,j}(t),
    \end{eqnarray*}
where $(a)$ follows by reverse triangle inequality and $(b)$ follows because $\cE_t$ holds. Since for any $i,j\in\bA$, $\M(i,j)=-\m(i,j)$ and $\Mh(i,j,t)=-\mh(i,j,t)$, it follows that 
\begin{eqnarray*}
   \lvert \m(i,j) - \mh(i,j,t)\lvert &=& \lvert \M(i,j) - \Mh(i,j,t) \lvert  \\
   &\leq& \beta_{i,j}(t). 
\end{eqnarray*}
\end{proof}

\subsection{Proof of \autoref{lem:sampl-complex-eps}}
By \autoref{lem:stoppingcond}, we have $\mh(b_t, c_t,t) \leq \beta_{b_t, c_t}(t)$ or equivalently \begin{equation}\Mh(b_t,c_t,t) \geq  - \beta_{b_t, c_t}(t)\;.\label{eq:step1}\end{equation} Then, knowing that $b_t \notin \OPT^{\eps_1}(t)$, there exists an arm $j$ such that $\Mh_{\eps_1}(b_t,j,t) = \eps_1 + \Mh(b_t,j,t) \leq \beta_{b_t, j}(t)$. Using further the definition of $c_t$, it follows that $\eps_1 + M(b_t,c_t,t) \leq \beta_{b_t, c_t}(t)$. Combining this with inequality \eqref{eq:step1} yields $$\beta_{b_t, c_t}(t) > \eps_1/2.$$ 

\subsection{Proof of Lemma~\ref{lem:samplold}}
In this section assume $\cE_t$ holds. If $t<\tau_\delta^{\eps_1}$, then, $Z_1^{\eps_1}(t) \leq 0$ or $Z_2^{\eps_1}(t) \leq 0$. We will analyze  the 4 different cases that could happen. %Recall that $k_t := \argmax_{i \in \{b_t, c_t\}} \beta_{i}(t)$. 
\paragraph{Case 1.1:} $b_t$ is a Pareto optimal arm. 
From the definition of the gap of an optimal arm and using \autoref{lem:gap_opt} it follows 
$\Delta_{b_t} \leq \Mh(b_t, c_t)$ which on $\cE_t$ and using \autoref{lem:existence_dom} yields 
\begin{equation}
  \Delta_{b_t}  + \eps_1 \leq \Mh(b_t,c_t, t) + \beta_{b_t, c_t}(t) + \eps_1 % \textcolor{red}{\leq} 4\beta_{b_t}(t), 
\end{equation}
then, noting that there exists $j \in \bA\setminus\{ b_t\}$ such that $\Mh(b_t, j,t) + \eps_1 \leq \beta_{b_t, j}(t)$ and by definition of $c_t$, we have 
\begin{equation}
 \Mh(b_t, c_t, t)+ \eps_1 \leq \beta_{b_t, c_t}(t),
\end{equation}
therefore, 
\begin{eqnarray*}
    \Delta_{b_t} + \eps_1 &\leq&  2(\beta_{b_t, c_t}(t).%\\
    %&\leq& 4 \beta_{b_t}(t).
\end{eqnarray*}
%\todoe{Je n'ai pas compris le cas 1.1, et comment tu utilises le Lemma 6}

\paragraph{Case 1.2:} $b_t$ is a sub-optimal arm. By definition of $c_t$ and using $\M=-\m$, we have 
\begin{align}
 c_t &\in \argmax_{j\in \bA \setminus\{ b_t\}}  \mh(b_t, j, t) + \beta_{b_t, j}(t), 
\end{align}
then, from the definition of the gap of a sub-optimal arm and since $\cE_t$ holds, we know that there exists an arm $b_t^\star$ such that 
\begin{eqnarray*}
    \Delta_{b_t} = \m(b_t, b_t^\star) &\leq&\mh(b_t, b_t^\star, t) + \beta_{b_t, b_t^\star}(t),\\
    &\overset{(a)}{\leq}& \mh(b_t, c_t, t) + \beta_{b_t, c_t}(t), \\
    &\overset{(b)}{\leq}& 2\beta_{b_t, c_t}(t).% \\
    %&\leq& 4\beta_{b_t}(t).
\end{eqnarray*}
where $(a)$ uses the definition of $c_t$ and $(b)$ uses Lemma~\ref{lem:stoppingcond}.
%\todoe{Ce cas me semble correct (j'ai rajouté quelques détails).}
\paragraph{Case 2.1:} $c_t$ is a Pareto optimal arm. If $b_t$ is an optimal arm,  it follows that $\Delta_{c_t}\leq \Mh(b_t, c_t)$ which on $\cE_t$ yields $\Delta_{c_t}\leq \Mh(b_t, c_t, t) + \beta_{b_t, c_t}(t)$, then, similarly to case 1.1, we have $\Mh(b_t, j,t) + \eps_1 \leq \beta_{b_t, j}(t)$  so $$\Delta_{c_t} + \eps_1 {\leq} 2 \beta_{b_t, c_t}(t).$$ Assume $b_t$ is a sub-optimal arm. Then, $\Delta_{c_t} \leq \Mh(b_t, c_t)^+ + \Delta_{b_t}$. Using a similar reasoning as in case 1.2, it holds that $\Delta_{b_t}\leq \mh(b_t, c_t, t) + \beta_{b_t, c_t}(t)$, so
%we consider two sub-cases: (i) $b_t^\star \notin \tm{U}^{b_t}_t$ and (ii) $b_t^\star \in \tm{U}^{b_t}_t$. If $b_t^\star \notin \tm{U}^{b_t}_t$, then using Lemma~\ref{lem:smplemmadom} $\Delta_{b_t} < 2\beta_{b_t}(t) \leq 2\beta_{c_t}(t)$ so, 
\begin{eqnarray*}
    \Delta_{c_t}&\leq& \M(b_t, c_t)^+ + \Delta_{b_t},\\
    &\leq& (\Mh(b_t, c_t, t) + \beta_{b_t, c_t}(t))^+  + \mh(b_t, c_t,t)+ \beta_{b_t, c_t}(t),\\
    &=& (-\mh(b_t, c_t, t) + \beta_{b_t, c_t}(t) )^+  + \mh(b_t, c_t,t)+ \beta_{b_t, c_t}(t), \\
    &\overset{(a)}{\leq}& \max(2\beta_{b_t, c_t}(t), \mh(b_t, c_t,t)+ \beta_{b_t, c_t}(t)) \\
    &\overset{(b)}{\leq}& 2\beta_{b_t, c_t}(t).% \\
    %&\leq& 4\beta_{c_t}(t), 
\end{eqnarray*}
where $(a)$ follows from $(x-y)^+  + (x + y) \leq \max(x+y, 2x)$ and $(b)$ follows from $\mh(b_t, c_t, t)\leq \beta_{b_t, c_t}(t)$ (\autoref{lem:stoppingcond}). 
%If $b_t^\star \in \tm{U}^{b_t}_t$, then $\Delta_{c_t} \leq \m(b_t, c_t, t) + \beta_{b_t}(t) + \beta_{c_t}(t)$, and $\M(b_t, c_t, t) < \beta_{c_t}(t) - \beta_{b_t}(t)$ (since $c_t \in \tm{U}^{b_t}_t$). Thus, 
%\begin{align*}
%    \Delta_{c_t}&\leq \M(b_t, c_t)^+ + \Delta_{b_t}\\
%    &\leq (\M(b_t, c_t, t) + \beta_{b_t}(t) + \beta_{c_t}(t))^+ + \m(b_t, c_t, t) + \beta_{b_t}(t) + \beta_{c_t}(t)\\
%    &\leq (\beta_{c_t}(t) - \beta_{b_t}(t) + \beta_{b_t}(t) + \beta_{c_t}(t))^+ + 2(\beta_{b_t}(t) + \beta_{c_t}(t))\\
%    &\leq 6\beta_{c_t}(t). 
%\end{align*}
%\todoe{Un truc non compris dans le cas 2.1}
\paragraph{Case 2.2:} $c_t$ is a sub-optimal arm. We know that there exists an arm $c_t^\star$ such that $\Delta_{c_t} = \m(c_t, c_t^\star)$. It $c_t^\star = b_t$ then, since $\m(j,i) \leq \M(i,j)$ (follows from the definition), we have 
\begin{eqnarray*}
    \Delta_{c_t} =\m(c_t, c_t^\star) &=& \m(c_t, b_t),\\
    &\leq& \M(b_t, c_t), \\
    &\overset{(a)}{\leq}& \Mh(b_t, c_t, t) + \beta_{b_t, c_t}(t), \\
 &\overset{(b)}{\leq}& 2\beta_{b_t, c_t}(t), 
\end{eqnarray*}
where $(a)$ follows from $\cE_t$ and $(b)$ has been already justified in the case 1.1. If  $b_t\neq c_t^\star$, then by definition of $c_t$, we have 
$$ \mh(b_t, c_t, t) + \beta_{b_t, c_t}(t) \geq \mh(b_t, c_t^\star, t) + \beta_{b_t, c_t^\star}(t),$$
which implies that there exists $d\in [D]$ such that 
$$ \muh_{c_t}^d(t) - \muh_{b_t}^d(t) + \beta_{b_t, c_t}(t) \geq \muh_{c_t^\star}^d(t) - \muh_{b_t}^d(t) + \beta_{b_t, c_t^\star}(t) \overset{\cE_t}{\geq} \mu_{c_t^\star}^d - \mu_{b_t}^d,$$
then, 
$$ \mu_{c_t}^d - \mu_{b_t}^d + 2\beta_{b_t, c_t}(t) \overset{\cE_t}{\geq} (\muh_{c_t}^d(t) - \muh_{b_t}^d(t) - \beta_{b_t, c_t}(t)) + 2\beta_{b_t, c_t}(t) \geq \mu_{c_t^\star}^d - \mu_{b_t}^d.$$
Put together, there exists $d\in [D]$ such that 
\begin{eqnarray*}
\mu_{c_t^\star}^d - \mu_{c_t}^d \leq  2\beta_{b_t, c_t}(t),
\end{eqnarray*}
so $$ \Delta_{c_t} = \min_d (\mu_{c_t^\star}^d - \mu_{c_t}^d) \leq 2\beta_{b_t, c_t}(t),$$
which achieves the proof of the lemma. 
%If $c_t^\star \notin \tm{U}^{c_t}_t$, by \autoref{lem:smplemmadom}, $\Delta_{c_t} \leq 2\beta_{c_t}(t)$. In the sequel, assume $c_t^\star \in \tm{U}^{c_t}_t$, that is for all $d$, 
%\begin{equation}
%    \muh_{c_t}^d(t) + \beta_{c_t}(t)  < \muh_{c_t^\star}^d(t) + \beta_{c_t^\star}(t), 
%\end{equation}
%so it holds that 
%\begin{equation}
%\label{eq:absurd1}
%  \m(b_t, c_t, t)+ \beta_{c_t}(t) < \m(b_t, c_t^\star, t)+ \beta_{c_t^\star}(t), 
%\end{equation}
%\begin{equation}
%\label{eq:absurd1}
%  \Mh(b_t, c_t, t) - \beta_{c_t}(t) > \Mh(b_t, c_t^\star, t) - \beta_{c_t^\star}(t), 
%\end{equation} which by definition of $c_t$, is impossible unless $c_t^\star = b_t$. 
%On the other hand, if $\tm{U}^{b_t}_t= \emptyset$, then \eqref{eq:absurd2} is impossible unless $c_t^\star = b_t$. 
%Put together, if $c_t^\star \in \tm{U}^{c_t}_t$, then $b_t = c_t^\star$ so that on $\cE_t$, $\Delta_{c_t} \leq \m(b_t, c_t, t) + \beta_{b_t}(t) + \beta_{c_t}(t)\leq 4\beta_{c_t}(t)$, where the last step uses Lemma~\ref{lem:stoppingcond}. 
%\todoe{Ce cas me semble correct}

\subsection{Proof of \autoref{thm:sampcompl}}
\begin{proof}[Proof of \autoref{thm:sampcompl}]
    Using \autoref{lem:sampl-complex-eps}, \autoref{lem:samplwm} and \autoref{lem:samplold}, we have that, if \algname has not stopped during round $t$ and the event $\cE_t$ holds, then 
    \begin{enumerate}[a)]
        \item $\omega^k\leq 2\beta_{b_t, c_t}(t)$ (\autoref{lem:samplwm}), 
        \item $\eps_1 \leq 2\beta_{b_t, c_t}(t)$ (\autoref{lem:sampl-complex-eps}),  
        \item $\Delta_{b_t}\leq 2\beta_{b_t, c_t}(t)$ and $\Delta_{c_t}\leq 2\beta_{b_t, c_t}(t)$(\autoref{lem:samplold})
    \end{enumerate}
    hold simultaneously. Which yields
    \begin{eqnarray}
        \tau_\delta \ind_{\cE} &\leq& \sum_{t=1}^\infty \ind{\{\max(\omega^k, \eps_1, \Delta_{k_t}) \leq 2 \beta_{k_t, k_t}(t)\}}\\
        &=& \sum_{t=1}^\infty \ind{\{\Delta_{k_t}^{k, \eps_1} \leq 2 \beta_{k_t, k_t}(t)\}}\\
        &=& \sum_{t=1}^\infty \sum_{a=1}^K\ind{\{\{\Delta_{a}^{k, \eps_1} \leq 2 \beta_{a, a}(t)\} \land \{k_t = a\}\}}\\
        &=&  \sum_{a=1}^K \sum_{t=1}^\infty \ind{\{\{\Delta_{a}^{k, \eps_1} \leq 2 \beta_{a, a}(t)\} \land \{k_t = a\}\}} \\
        &=& \sum_{a=1}^K \sum_{t=1}^\infty (T_a(t+1) - T_a(t))\ind{\{\{\Delta_{a}^{k,\eps_1} \leq 2 \beta_{a, a}(t)\} \}} \\
        &\leq& \sum_{a=1}^K \inf\{s\in \bN^\star: \Delta^{k, \eps_1} > 2 \beta_{a, s} \}. 
    \end{eqnarray}
Then, \autoref{lem:bound_inv_beta_ek} yields, 
$$ \inf\{s\in \bN^\star: \Delta_a^{m, \eps_1} > 2 \beta_{a, s}\} \leq  \frac{8\times 16\sigma^2}{(\Delta_a^{m, \eps})^2}\log(\frac{2}{\delta}\log(\frac{8\times 16 \sigma^2}{(\Delta_a^{m, \eps})^2})).$$
Therefore, 
\begin{equation}
   \tau_\delta \ind_{\cE} \leq \sum_{a \in \bA} \frac{128\sigma^2}{(\Delta_a^{m, \eps})^2}\log\left(\frac{2}{\delta} \log\left(\frac{128\sigma^2}{(\Delta_a^{m, \eps})^2}\right)\right) . 
\end{equation}
\end{proof}
%\subsection{When $k$ is given to \algname}
%\label{subsec:k-param-of-ape}
\section{Algorithm for the$-\veps_2-$relaxation}
\label{sec:alg_eps_2}
In this section, we analyse the sample complexity of \algname when it is associated to the stopping time  $\tau_{\delta}^{\eps_1, \eps_2}$ for identifying an $(\eps_1, \eps_2)-$cover of the \emph{Pareto set}.  The sampling rule remains unchanged an we prove that the algorithm does not require more samples to find an $(\eps_1, \eps_2)-$covering than to find the \emph{Pareto set}. Furthermore, we assess the performance of \algname through empirical evaluation.  
In appendix bb, we the analyze the sample complexity of 
\algname for the $(\eps_1, \eps_2)-$PSI problem and appendix shows an empirical study of this sample complexity. 
\subsection{Theoretical  analysis}
We recall the definition of \algname. 

\begin{algorithm}[H]
\caption{Adaptive Pareto Exploration}\label{alg:three}
\KwData{parameter $\eps_1\geq 0$}
%\KwResult{The \emph{Pareto set} $\cS^\star$ or a relaxed subset}
\Input{sample each arm once, set $t=K$, $T_i(t)=1$ for any $i\in \bA$} 
 \For{$t=1,2,\dots$}{
  $b_t := \argmax_{i \in \bA \setminus \OPT^{\eps_1}(t)} \min_{j \neq i }\Mh^+(i,j,t)$\;
     $c_t := \argmin_{j\neq b_t} \Mh^{-}(b_t, j, t)$\;

  \Sample{$b_t$ and $c_t$}\;
  $t \gets t + 1$\;
 }
 %\Output{$\cO_{\tau_\delta}$}
\end{algorithm}
We recall the stopping rule $\tau_\delta^{\eps_1, \eps_2}$. 
\paragraph{Stopping rule.} Let $\eps_1, \eps_2\geq 0$ and  $0<\delta<1$, then 
\begin{equation}
\label{eq:stopping-rule}
	\tau_\delta^{\eps_1, \eps_2}:= \inf \{ t\in \bN^\star:\;  \tilde Z_1^{\eps_1, \eps_2}(t) > 0 \; \land   \tilde Z_2^{\eps_1, \eps_2}(t) > 0\},
\end{equation}
where,
\begin{eqnarray*}
\tilde Z_1^{\eps_1, \eps_2}(t) &:=& \min_{i \in S(t)}  \max(g_i^{\eps_2}(t), h_i^{\eps_1}(t))\\
\tilde Z_2^{\eps_1, \eps_2}(t) &:=& \min_{i \in S(t)^{\complement}}  \max(g_i^{\eps_2}(t), h_i^{\eps_1}(t)),
\end{eqnarray*}
and
\begin{eqnarray*}
  g_i^{\eps_2}(t) &:=& \max_{j \in \bA \setminus\{i\}}  \mh^-(i,j,t)  + \eps_2 \ind\{j \in \OPT^{\eps_1}(t)\} 
  \\
  h_i^{\eps_1}(t) &:=& \min_{j\in\bA\setminus\{i\}}\Mh^-(i,j,t)+\eps_1 
\end{eqnarray*}
\paragraph{Recommendation rule.} When 
it is associated to the stopping time $\tau_\delta^{\eps_1, \eps_2}$, \algname recommends
$$\cO_{\tau_\delta^{\eps_1, \eps_2}} := \OPT^{\eps_1}(\tau_\delta^{\eps_1, \eps_2})
%S({\tau_\delta}) \cup \{ i \in S(\tau_\delta)^\complement:  g_i^{\eps_2}(t) < 0 \}
,$$ which can be understood as follows. When \algname stops, the arms not yet identified as (nearly) optimal are either $\eps_2-$dominated by an arm in $\OPT^{\eps_1}(\tau_\delta^{\eps_1, \eps_2})$ or sub-optimal, which is proven formally in \autoref{lem:correctness-eps1-eps-2-cover}. 
% finalement preuve generrique
\begin{lemma}
\label{lem:correctness-eps1-eps-2-cover}
    Fix $\delta \in (0, 1), \eps_1, \eps_2 \geq0$ then \algname associated to the stopping time $\tau_\delta^{\eps_1,\eps_2}$ recommends an $(\eps_1, \eps_2)-$cover of the \emph{Pareto set} on the event $\cE$.  \end{lemma}
    \begin{proof}
Assume $\cE$ holds. Let  $t=\tau_\delta^{\eps_1, \eps_2}$ and $i\in \OPT^{\eps_1}({t})$. For any $j\neq i$, $ \M(i,j) + {\eps_1}\overset{\cE}{\geq}\Mh^-(i,j,t) + {\eps_1}> 0$ that is $i \in \cS^\star_{\eps_1}$. Therefore, on the event $\cE$, $\OPT^{\eps_1}({t})\subset \cS^\star_{\eps_1}$. When \algname stops -associated to the stopping time $\tau_\delta^{\eps_1, \eps_2}$-, $\tilde Z^{\eps_1, \eps_2}_1(t) > 0$ and $\tilde Z^{\eps_1, \eps_2}_2(t) >0$. 
 Under this condition, $$\OPT^{\eps_1}(t)\neq \emptyset.$$ Indeed, since $Z^{\eps_1, \eps_2}_1(t)>0$ and $\tilde Z^{\eps_1, \eps_2}_2(t)>0$, if $\OPT^{\eps_1}(t) = \emptyset$ then, by the stopping rule, for any arm $i$, $h_i^{\eps_1}(t)<0$  and $g_i^{\eps_2}(t)>0$. That is, for any arm $i$, 
      $$\exists j\neq i \tm{ such that } \m(i,j)\overset{\cE}{>} \mh^-(i,j,t)>0,$$ so every arm is strictly dominated, which is impossible since the \emph{Pareto set} cannot be empty. Then, $\OPT^{\eps
_1}(t)\neq \emptyset$ and 
    for any $i\in \cO_t^\complement
 = \OPT^{\eps_1}(t)^\complement$, by the stopping rule it holds that $\max(g_i^{\eps_2}(t), h_i^{\eps_1}(t)) > 0$ and noting that $h_i^{\eps_1}(t)<0$ since $i\notin \OPT^{\eps_1}(t)$ we have $g_i^{\eps_2}(t)>0$, that is $$ \mh^-(i,j,t)  +  \eps_2 \ind\{j \in \cO_t\} >0,$$
 which on the event $\cE$ yields 
 $$ \m(i,j) + \eps_2 \ind\{j \in \cO_t\}  >0.$$
 Therefore, either
    \begin{enumerate}[i)]
    \item $\exists j \in \bA \tm{ such that } \m(i,j)>0$ that is $\vmu_i \prec \vmu_j$ or 
    \item $\exists j \in \cO_{t}$ 
    \tm{ such that } $\m(i,j) + \eps_2 > 0$ that is $\vmu_i \prec \vmu_j + \mathbf{\eps_2}$ with $\mathbf{\eps_2}:= (\eps_2, \dots, \eps_2)$. 
        %\item $\forall\; i \notin \cO_t, \; j \in \cO_t \tm{ such that } \vmu_i \prec \vmu_j + \eps_2$, and 
        %\item $\cO_t \subset \cS_{\eps_1}^\star,$
    \end{enumerate}
Put together, $\cO_t \subset \cS^\star_{\eps_1}$ and  for any $i\notin \cO_t$, either $i \notin \cS^\star$ ($i$ is a sub-optimal arm) or there exists $j\in \cO_t$ such that $\vmu_i \prec \vmu_j + \mathbf{\eps_2}$. Thus is $\cO_t$ is an $(\eps_1, \eps_2)-$cover of the \emph{Pareto set} and \algname associated to the stopping time $\tau_\delta^{\eps_1, \eps_2}$ is correct for an $(\eps_1, \eps_2)-$cover identification. 
\end{proof}
The following lemma, which is similar to \autoref{lem:stoppingcond} will be used to prove that  on the event $\cE$, $\tau_\delta^{\eps_1, \eps_2} \leq \tau_\delta^{\eps_1}$. 
\begin{lemma}
\label{lem:stoppingcond2}
       During round $t$, if $t<\tau_\delta^{\eps_1, \eps_2}$ then for any $i\in \bA$, $\mh(b_t,j,t) \leq \beta_{b_t, j}(t).$ 
       %$\tilde Z_1(t) \leq 0 $ or $\tilde Z_2(t) \leq 0$, 
       \begin{proof}
       Recall that by definition $t<\tau_\delta^{\eps_1, \eps_2}$ implies that 
       $\tilde Z_1^{\eps_1, \eps_2}(t) \leq 0 $ or $\tilde Z_2^{\eps_1, \eps_2}(t) \leq 0$. 
           By definition of $b_t$ and noting that $\M(i,j) = -\m(i,j)$, we have 
           \[ b_t \in \argmin_{i\in \OPT^{\eps_1}(t)^\complement} \max_{j\neq i }\mh(i,j,t) - \beta_{i,j}(t).\]
so that if there exists $j$ such that $\mh(b_t,j,t)>\beta_{b_t, j}(t)$, we would have 
$$ \max_{j\neq b_t } \mh(b_t, j,t) - \beta_{b_t, j}(t) >0.$$
Then, 
\begin{equation}
 \forall i \in \OPT^{\eps_1}(t)^\complement\;, 0<\max_{j\neq i}\mh(i,j,t) - \beta_{i,j}(t)\leq g^{\eps_2}_i(t).   
\end{equation}
Furthermore, since we have 
\begin{equation}
    \forall i \in \OPT^{\eps_1}(t)\;, h^{\eps_1}_i(t) >0, 
\end{equation}
it comes that for any $i$, $\max(h^{\eps_1}_i(t), g^{\eps_2}_i(t))>0$ which imply that $\tilde Z^{\eps_1, \eps_2}_1(t)>0$ and $\tilde Z^{\eps_1, \eps_2}_2(t)>0$. Therefore, 
for any $i\in \bA, \mh(b_t,j,t)\leq \beta_{b_t, j}(t)$. 
       \end{proof}
\end{lemma}
We recall the following lemma which does not depend on the stopping time. 

\begin{lemma}
\label{lem:sampl-complex-eps_1-eps_2}
    During round $t$, if the algorithm has not stopped then $\beta_{b_t, c_t}(t) > \eps_1/ 2$. 
\end{lemma}
Noting that the proof of \autoref{lem:samplold} can be derived from  the conditions \begin{enumerate}[a)]
    \item $\forall j,\; \mh(b_t, j, t)\leq \beta_{b_t, j}(t)$,
    \item $\exists j\neq b_t$ such that $\Mh(b_t, j,t) + \eps_1 \leq \beta_{b_t, j}(t),$
\end{enumerate}
which also holds by \autoref{lem:stoppingcond2}) and the definition of $b_t, c_t$. Therefore, the following lemma also holds when \algname is associated to the stopping time $\tau_\delta^{\eps_1, \eps_2}$. 
\begin{lemma}
\label{lem:samplold2}
    During round $t$, if $\cE_t$ holds and  $t<\tau_\delta^{\eps_1, \eps_2}$ then $\Delta_{b_t} \leq 2 \beta_{b_t, c_t}(t)$ and $\Delta_{c_t} \leq 2 \beta_{b_t, c_t}(t)$.%, where $k_t$ is the least sampled arm among $b_t$ and $c_t$.
\end{lemma}
Put together, \autoref{lem:correctness-eps1-eps-2-cover}, \autoref{lem:sampl-complex-eps_1-eps_2}, \autoref{lem:samplold2} yields the following theorem.
% TODO remplacer par le theoreme final. 
\begin{theorem}
\label{thm:sampcompl2}
Fix $\delta \in (0, 1)$, $\eps_1, \eps_2 \geq 0$. Then \algname associated to the stopping time $\tau_{\eps_1, \eps_2}$ outputs an $(\eps_1, \eps_2)-$cover of the \emph{Pareto set} with probability at least  $1-\delta$ using at most the following number of samples,
%TODO remplacer avec les trucs
\begin{equation}
     \sum_{a \in \bA} \frac{88}{(\Delta_a^{\eps})^2} \log\left(\frac{K(K-1)D}\delta \log\left(\frac{12e}{\Delta^{\eps}_{a}}\right)\right),
\end{equation}
where $\Delta_a^{\eps} := \max(\Delta_a, \eps_1)$. 
\end{theorem}
This is the first gap-dependent sample complexity upper-bound for the $(\eps_1, \eps_2)-$cover of the {Pareto set}. In particular, it gives a gap-dependent sample complexity of $\eps-$accurate {Pareto set} identification \cite{zuluaga_e-pal_2016} which corresponds the particular case $\eps_1 = \eps_2 = \eps$ of the {Pareto set} cover.  Therefore, \algname associated to the stopping time $\tau_\delta^{\eps_1, \eps_2}$ is a competitor of $\eps-$PAL for $\eps-$ accurate {Pareto set} identification with gap-dependent guarantees. Moreover, we do not require the Gaussian smoothness assumption required in \cite{zuluaga_e-pal_2016}. 
While our sample complexity result does not clearly show the dependence in $\eps_2$ we not that for some problems, we have a nearly matching lower bound that does not depend on $\eps_2$. In particular, consider the case $D=1, \eps_1 = 0, \eps_2 >0$ an assume there is a unique optimal arm (classical assumption) $a_\star$. For this setting, an algorithm for $(\eps_1, \eps_2)-$cover is required to output a set $\hat S$ such that $\hat S \subset \cS^\star = \{ a_\star\}$ and for any $i\neq a_\star$ either $\mu_i < \mu_{a_\star}$ or $\mu_i \leq \mu_{a_\star} + \eps_2$ which trivially holds as long as $\hat S \subset \cS^\star$ therefore, this is just BAI. The lower bound of this problem is known and does not depend on $\eps_2$ (\cite{kaufmann_complexity_2014}). 
\begin{theorem}
\label{thm:lower_bound_eps_2}
 lower bound worst case dans le cas $\eps_2$.    
\end{theorem}

\section{Lower Bounds}
\label{sec:lower_bounds}
%TODO pas fini 
In this section, we give a gap-dependent lower-bound for the $k-$relaxation in some configurations. We use the change of distribution lemma of \cite{kaufmann_complexity_2014} (lemma 1). 
\begin{theorem}
    Let $K, D\geq 2$. There exists a bandit instance $\nu$ such that for $m \geq 1 \lor (\lvert \cS^\star\lvert - 2) $, for any $\delta-$correct algorithm $\cA$
    \[ \bE_\nu^{\cA}[\tau_\delta] \geq \frac{c}{D} \log\left(\frac1\delta\right) \sum_{k=1}\frac{1}{(\Delta_k^m)^2},\]
    where $\Delta_k^m := \Delta_k+ \omega^m$.
\end{theorem}
 \begin{proof} Let $p = \lvert \cS^\star\lvert$. 
        w.l.o.g assume $\cS^\star = \{1, \dots, p\}$ and $\cS^{\star,m} = \{1, \dots, m\}$. 
        Let $\vmu_1 \in \bR^D$ and for $(p-2)\leq i\leq p$, 
        $$ \mu_i^d := \begin{cases}
            \phantom{-}2^{p-i}\omega  &\tm{ if } $d = 1$\\
            -2^{p-i}\omega &\tm{ else if } $d = 2$ \\
            \phantom{-}\mu_0^d &  \tm{ else. }
        \end{cases},$$
        for $1\leq i\leq p-3$, 

        $$\mu_i^d := \begin{cases}
           \phantom{-}(4 +2i) \omega &\tm{ if } $d = 1$\\
             - (4 +2i)\omega &\tm{ else if } $d = 2$ \\
            \phantom{-}\mu_0^d &  \tm{ else. }
        \end{cases}$$
        and for $i>p$, 
        $$ \mu_i^d :=
            \mu_0^d - \alpha_i
     $$
     where $\alpha_i < \omega$ for any $i > p$. 

By direct calculation, for $1\leq i,j\leq p -3$,
$$\M(i,j) = \M(j,i) = 2\omega\lvert i - j\lvert ,$$ and for $p-2\leq i, j\leq p$, 
$$\M(i, j) = \M(j,i) = 2^p\omega\lvert 2^{-i} - 2^{-j}\lvert,$$
for $i\leq p-3$ and $(p-2)\leq j\leq p$, 
$$\M(i, j) = \M(j, i) = (4 + 2i - 2^{p-j})\omega \geq 2\omega.$$
Therefore, computing $\omega_i$ and $\delta_i^+$ for any $i\in [p]$ yields
\begin{eqnarray*}
    \delta_i^+ &:=& \min_{j\in [p]\backslash \{i\}}\min(\M(i,j), \M(j,i)),
\\
&=&  \begin{cases}
    \omega & \tm{ if } i=p,\\
    2^{p-i-1} \omega & \tm{ if } i \in \{p-2, p-1\} \\
    2\omega & \tm{ else, } 
\end{cases} 
\end{eqnarray*}
additionally, for any $i\leq p$, 
\begin{eqnarray*}
 \omega_i &:=& \min_{j\neq i} \M(i,j), \\ &=&  \begin{cases}
    \omega & \tm{ if } i=p,\\
    2^{p-i-1} \omega & \tm{ if } i \in \{p-2, p-1\} \\
    2\omega & \tm{ else.} 
\end{cases}   
\end{eqnarray*}
Thus,  $$\omega^{(p)} =\omega^{(p-1)} =  \omega \tm{ and }\omega^{(p-2)} = 2\omega.$$
Let $\gamma>0$, since $\M(i, i+1) = \M(i+1, i) = \delta_{i}^+$, 
$$ \vmu_i + \delta_i^+ + \gamma $$
Pareto dominates $\vmu_{i+1}$ or $\vmu_{i-1}$ and $\vmu_i - \delta_i^+ - \gamma \prec \vmu_{i+1} \tm{ or } \vmu_{i-1}$. Moreover, it is easy to observe that for $m \in \{p-2, p-1, p\}$ and any $i \in [p]$,
$$\vmu_{i} + \delta_i^+ + \omega^{(m)} + \gamma$$
Pareto dominates 1 (if $m\in \{p,p-1\}$)  or 2 (if $m=p-2$) other optimal arms. Letting $m\in \{p-2, p-1, p\}$, for any $i\in [p]$, we define the alternative bandit $\nu^{(i)}$ whose means are 
\begin{equation}
    \vmu^{(i)}_k = \begin{cases}
        \vmu_k & \tm{ if } k\neq i \\ \vmu_k - \delta_i^+ - \omega^{(m)} - \gamma & \tm{ if } k = i \tm{ and }\bP_\nu( k \in \hat S) \geq \frac12\\
         \vmu_k + \delta_i^+  +\omega^{(m)} - \gamma & \tm{ if } k = i \tm{ and } \bP_\nu( k \in \hat S) <\frac12.
    \end{cases}
\end{equation}
Therefore, since $\cA$ is $\delta-$correct, and by what precedes,
\begin{itemize}
    \item $\tm{ if }\bP_\nu(i \in \hat S) \geq \frac12 \tm{ then } \bP_{\nu^{(i)}}(i \in \hat S) \leq \delta$ and 
    \item $\tm{ if }\bP_\nu(i \in \hat S) <\frac12 \tm{ then } \bP_{\nu^{(i)}}(i\in \hat S) \geq 1-\delta$. 
\end{itemize}
The first point follows simply from the definition of $\delta_i^+$ and the fact that by design $\M(i,j) = \M(i, j)$ for $i,j\in [p],$ For the second point, if $m\in \{ p, p -1\}$, in the bandit $\nu^{(i)}$, at least one arm of $\cS^\star(\nu)$ is no longer optimal, then $\lvert \cS^\star(\nu^{(i)}) \lvert \leq p-1 \leq m.$ So $\bP_{\nu^{(i)}}(i\in \hat S)\geq 1-\delta$. If $m=p-2$ since now two arms of $\cS^\star(\nu)$ are now dominated, we have $\lvert \cS^\star(\nu^{(i)}\lvert \leq p-2 = m,$ hence $\bP_{\nu^{(i)}}(i\in \hat S)\geq 1-\delta$
Using lemma 1 of \cite{kaufmann_complexity_2014}, on the event $\cF_\tau-$measurable event $$E_i = \begin{cases}
    \{ i \in \hat S\} & \tm{ if } \bP_\nu(i\in \hat S)\geq \frac12, \\
    \{i \notin \hat S\} &\tm{ if } \bP_\nu(i\in \hat S)<\frac12,
\end{cases}$$
for which $\bP_\nu(E_i) \geq \frac12$ and $\bP_{\nu^{(i)}}(E_i)\leq \delta$, it comes that 
$$ \sum_{a\in \bA} \bE_\nu(T_a(\tau))\KL(\nu_a, \nu_a^{(i)}) \geq d(\bP_\nu(E_i), \bP_{\nu^{(i)}}(E_i)), $$
hence 
\begin{equation}
\label{eq:lemma_change_distrib}
 \bE_\nu(T_i(\tau))\KL(\nu_i, \nu_i^{(i)}) \geq d(\bP_\nu(E_i), \bP_{\nu^{(i)}}(E_i)),   
\end{equation}
where $d(x,y) = x\log(x/y) + (1-x)\log((1-x)/(1-y))$ is the binary relative entropy. Since $\bP_\nu(E_i)\geq \frac12$ and $\bP_{\nu^{(i)}}(E_i) \leq \delta$, 
\eqref{eq:lemma_change_distrib} yields (see \cite{kaufmann_complexity_2014}),
\begin{eqnarray*}
    \bE_\nu(T_i(\tau)) &\geq& \frac{1}{\KL(\nu_i, \nu_i^{(i)})} \frac12\left( \log\left(\frac{1}{2\delta}\right) + \log\left(\frac{1}{2(1-\delta)}\right)\right) \\
    &=& 
    \frac{1}{2\KL(\nu_i, \nu_i^{(i)})} \log\left( \frac{1}{\delta(1-\delta)}\right)\\
    &\geq& \frac{1}{2\KL(\nu_i, \nu_i^{(i)})} \log(1/\delta),
\end{eqnarray*}
where the last inequality follows from $x(1-x) \leq x$. 

     il vaut mieux une config ou pour tous les bras optimaux i * wm domine un autre bras 
     -> fixer que le gap m, m-1 et m-2 pour les bras optimaux
    \end{proof}
\section{Best Arm Identification}
\label{sec:bai}
In this section, we discuss the sample complexity and the performance of \algname associated to the stopping rule $\tau_{0}^1$ for BAI. Noting that when $D=1$, the {Pareto set} is just the \emph{argmax} over the means, BAI and PSI are the same for uni-dimensional bandits. For this setting we should expect algorithms for PSI to be competitive with existing algorithms for BAI when $D=1$. We will show that it is actually the case for \algname. Let $D=1$ and $\nu$ be a one-dimensional $K-$armed bandit. Letting $a_\star$ denote the unique optimal arm of $\cS^\star =\{a_\star\}$, one can easily check that the gaps defined for PSI matches the common notion of gaps for BAI. Indeed, for any $a\neq a_\star$,
\begin{eqnarray*}
\Delta_{a}  &:=& \max_{j \in \cS^\star} \m(a, j), \\
&=& \m(a, a_\star) \\
&=&\mu_{a_\star} - \mu_a,
\end{eqnarray*}
and $$\Delta_{a_\star}  = \min_{j\neq a_\star} \Delta_j,$$
which matches the definition of the gap in the one-dimensional bandit setting (\cite{audibert_best_2010, kaufmann_complexity_2014}). Therefore, the sample complexity of \algname for BAI can be deduced from \autoref{thm:sampcompl}. 
\begin{theorem}
\label{thm:sampl_compl_BAI}
Let $\delta \in (0, 1), K\geq 2$ and $\nu$ a $K-$armed bandit with a unique best arm $a_\star$ and $1-$subgaussian distributions. \algname associated to be stopping time $\tau_0^k$ identifies the best arm $a^\star$ with probability at least $1-\delta$ using at most the following number of samples  \[ 
\sum_{a=1}^K \frac{88}{\Delta_a^2} \log\left(\frac{K(K-1)}\delta \log\left(\frac{12e}{\Delta_{a}}\right)\right). 
\]
\end{theorem}
In particular, $k$ is not meaningful in this setting. Under the unique optimal arm assumption, the algorithm will always stops when the best arm have been identified. And we have from the definition of $\omega_i$'s 
$$ \omega_1 := \min_{j\neq a_\star}\M(a_\star, j) = \min_{j\neq a_\star} \Delta_j = \Delta_{a_\star} \quad \text{ and } \quad \forall i\neq a_\star, \quad \omega_i < 0,$$
so for any $k\leq K$, $\max(\omega_k, \Delta_a) = \Delta_a$ which translates the fact that $k$ is not meaningful in this setting.
\begin{remark}
\label{rmk:improve_ape_for_BAI}
\autoref{thm:sampl_compl_BAI} could be improved. On the event $\cE$ we consider that for any pair of arms the difference of their empirical mean does not deviate too much from its actual value. For BAI, since we know that there is a unique optimal arm (enforced by assumption), it is sufficient to control the different between the best arm and any other arm, therefore we could replace $K(K-1)/2$ term due to union bound in the confidence bonus by $K-1$ and we could show that this will reflect in the sample complexity by replacing $K(K-1)$ by $2(K-1)$. However, this cannot be done in general for PSI since we don't known in advance the number of optimal arms. 
    % could be improved by using confidence interval on K-1 pairs and explain that we can't for general PSI 
\end{remark}
When $D=1$,  \algname reduces to sample at each round $t$, the least sampled among 
\begin{eqnarray}
\label{eq:sampling-rule-BAI}
    b_t &:=& \argmax_i \left\{\max_{j\neq i}U_{i,j}(t)\right\},\\
    c_t &:=& \argmin_{j\neq b_t} L_{b_t, j}(t),
\end{eqnarray}
where $U_{i,j}(t) := \muh_i(t) - \muh_j(t) + \beta_{i,j}(t)$ and $L_{i,j}(t):= \muh_i(t) - \muh_j(t) - \beta_{i,j}(t)$ are upper and lower bounds on  the difference $\mu_i - \mu_j$. To be in the same setting as LUCB and UGapEc which uses confidence interval on single arms, we would have $\beta_{i,j}(t) := \beta_{i}(t) + \beta_{j}(t)$, where $\beta_{i}'s$ are confidence bonuses on single arms such that $L_i(t) := \muh_i(t) - \beta_{i}(t)$ and $U_i(t):= \muh_i(t) + \beta_i(t)$ are lower and upper confidence bounds on $\mu_i$. Then \eqref{eq:sampling-rule-BAI} rewrites as 
\begin{eqnarray*}
    b_t &:=& \argmax_i \left\{U_i(t) -\max_{j\neq i}L_{j}(t)\right\},\\
    c_t &:=& \argmax_{j\neq b_t} U_j(t),
\end{eqnarray*}
%where $L_i(t) := \muh_i(t) - \beta_{i}(t)$ and $U_i(t):= \muh_i(t) + \beta_i(t)$. 
This resembles the sampling rule of UGap, which defines 
\begin{eqnarray}
    b_t^{\text{UGap}} &:=& \argmax_{i} \left\{L_i(t)-\max_{j\neq i} U_j(t) \right\}, \\
    c_t^{\tm{UGap}} &:=& \argmax_{j\neq b_t} U_i(t),
\end{eqnarray}
and pull the least sampled so far. Moreover, how algorithm could be analyzed were both $b_t, c_t$ (in the spirit of LUCB \cite{kalyanakrishnan_pac_2012}) are sampled using the same arguments employed in the proof of \autoref{thm:sampcompl}. The following lemma proves that for $D=1$, the stopping time $\tau_{0}$ is close to the one of LUCB or UGap. 
In the sequel, for this section, we remove the dependence in $\eps_1$ to write $Z_i(t)$ instead of $Z_i^{0}$ for $i\in \{0, 1\}$. 
\begin{lemma}
\label{lem:stoptimeequal}
    Let $\delta \in (0,1)$. For $D=1$,  
    $$\inf\{{t\in \bN^\star : Z_1(t)>0} \land Z_2(t) >0 \} = \inf\{t\in \bN^\star : \muh_{b_t}(t) - \beta_{b_t}(t) > \muh_{c_t}(t) + \beta_{c_t}(t) \}.$$
\end{lemma}
   \begin{proof}
       Let $S(t) = \{\hat a_t\}$. $Z_1(t)$ and $Z_2(t)$ simplifies to  
        \begin{eqnarray}
            Z_1(t) &=&  L_{\hat a_t}(t) - \max_{j\neq \hat a_t} U_j(t), 
        \\ Z_2(t) &=& \min_{i \neq \hat a_t} \{ \max_{j\neq i } L_j(t) - U_i(t)\}. 
        \end{eqnarray}
        We can observe that  $$ Z_1(t) > 0 \equi Z_2(t) > 0.$$
        Indeed, 
        \begin{eqnarray}
         Z_1(t) > 0 &\impl& \forall i\neq \hat a_t, L_{\hat a_t}(t) > U_i(t) \\
         &\impl& Z_2(t) >0. 
        \end{eqnarray}
        On the other side, 
        \begin{eqnarray}
            Z_2(t) > 0 &\impl& \forall i \neq \hat a_t ,\;\exists j\neq i \tm{ such that  }  L_j(t) - U_i(t)>0 \\
            &\impl& \hat a_t =  \argmax_i L_i(t) \tm{ and } \forall i\neq \hat a_t,\; L_{\hat a_t}(t) - U_i(t) >0,\\&\impl& 
            Z_1(t) >0. 
        \end{eqnarray}
        Now we will show that $$ Z_1(t) > 0 \equi \muh_{b_t}(t) - \beta_{b_t}(t) > \muh_{c_t}(t) + \beta_{c_t}(t).$$
    We have
    \begin{eqnarray}
        Z_1(t) > 0 &\impl& L_{\hat a_t}(t) > \max_{i\neq \hat a_t} U_i(t)\\ &\impl& \forall i\neq \hat a_t, U_i(t) - \max_{j\neq i } L_j(t) < 0, \\
        &\impl& b_t = \hat a_t,
    \end{eqnarray}
    where the last result follows by definition of $b_t$ and the fact that $$ U_{\hat a_t}(t) - \max_{i\neq \hat a_t} L_i(t) \geq L_{\hat a_t}(t) - \max_{i\neq \hat a_t} U_i(t) >0.$$
    Therefore, 
    \begin{eqnarray}
     Z_1(t) > 0 &\impl& b_t = \hat a_t \tm{ and } L_{\hat a_t}(t) - U_{c_t}(t) >0, \\&\impl&\muh_{b_t}(t) - \beta_{b_t}(t) > \muh_{c_t}(t) + \beta_{c_t}(t).   
    \end{eqnarray}
Similarly, 
\begin{eqnarray}
  \muh_{b_t}(t) - \beta_{b_t}(t) > \muh_{c_t}(t) + \beta_{c_t}(t) &\impl& \hat a_t = b_t \tm{ and }\forall i \neq \hat a_t,\; L_{\hat a_t} > U_{i}(t) \\
  &\impl& Z_1(t) > 0,
\end{eqnarray}
hence it holds that \begin{equation}
    Z_1(t)>0\land Z_2(t) >0 \equi   \muh_{b_t}(t) - \beta_{b_t}(t) > \muh_{c_t}(t) + \beta_{c_t}(t).
\end{equation}
    \end{proof}
Thus, for $D=1, \eps_1 = 0$ and using the stopping time $\tau_{\eps_1=0}$, \algname and UGap only differ in the  definition of $b_t$ and their stopping rules are close to LUCB. 
\paragraph{Experiments:} We evaluate the performance of \algname for BAI on two instance: one easy with $K=5$ and the second more difficult and with $K=10$. We use the instanciation of \algname with confidence bonuses on pair of arms \emph{but without the possible improvement invoked in \autoref{rmk:improve_ape_for_BAI}}. 
UGap and LUCB are implemented with the tightest known (to our knowledge) confidence bonus taken from \cite{katz-samuels_top_2019} (in spirit of the finite-time \emph{law of the iterated logarithm}\cite{jamieson_lil_2013}). LUCB++ is used with the improved confidence bonus given in \cite{simchowitz_simulator_2017}.
We set $\delta=0.01$ and the results are averaged over $5000$ independent trials. 
\autoref{fig:appx-F-results-bai} shows that \algname outperforms, LUCB, LUCB++ and UGap on both instances. We represent on the \texttt{y-axis} the sample complexity in units of the lower bound of BAI (\cite{kaufmann_complexity_2014}) : 
$$ H\log(1/2.4\delta) = \log(1/2.4\delta) \sum_{i=1}^K \frac1{\Delta_i^2}.$$
\begin{figure}[H]
     \centering
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
    \includegraphics[width=\textwidth]{data/F/bai_compare_boxplot_ape_5.png}
         \caption{$H =56.56 $}
         \label{fig:appx-F-results-bai-1}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
    \includegraphics[width=\textwidth]{data/F/bai_compare_boxplot_ape_10.png}
         \caption{$H = 381.78$}
         \label{fig:appx-F-results-bai-2}
     \end{subfigure}
        \caption{Empirical sample complexity expressed in units of the lower bound $H\log(1/2.4\delta)$ (blue line) on a random instance with $K=5$ (left)  and $K=10$ (right), $\delta=0.01$.}
        \label{fig:appx-F-results-bai}
\end{figure}
% TODO potentiellement le retirer. 
% \section{Comparison to LUCB$-k-m$}
% In this section, we compare the "at most m" optimal arms to the LUCB-k-m of \cite{chaudhuri_pac_2017}. Our setting differs from theirs in many points. The number of optimal arms is not known in advance. In \cite{chaudhuri_pac_2017}, the authors presented an algorithm whose sample complexity scales with $1/\tilde \Delta_i^2$ terms. Letting $\nu$ be a $K-$armed bandit and $D=1$ with means $\mu_1\geq \dots \geq  \mu_m > \mu_{m+1}\geq \dots\geq \mu_{K}$, then for any $k\in [K]$, 
% \begin{equation}
%     \tilde \Delta_{a} = \begin{cases}
%         \mu_a - \mu_{m+1} & \tm{ if } 1\leq a \leq k \\
%         \mu_k - \mu_{m+1} & \tm{ if } k+1\leq a\leq m \\
%         \mu_{m} - \mu_a & \tm{ if } k\geq m+1, 
%     \end{cases}
% \end{equation}
% which rewrites as 
% \begin{equation}
%     \tilde \Delta_{a} = \begin{cases}
%         \max(\mu_a - \mu_{m+1}, \mu_k - \mu_{m+1}) & \tm{ if } 1\leq a \leq m \\
%         \mu_{m} - \mu_a & \tm{ if } k\geq m+1,
%     \end{cases}
% \end{equation}
% where 
% $$\mu_k - \mu_m = \overset{k}{\argmax}_{i \in [m]} (\mu_i - \mu_m).$$
\section{Another Instanciation} 
\label{sec:another_instanciation}
In this section we derive an upper bound on the expectation of the sample complexity when the algorithm \algname is run with confidence bonuses similar to LUCB \cite{kalyanakrishnan_pac_2012}. This is different from \autoref{thm:sampcompl} for which the sample complexity is bounded only on the high-probability event $\cE$ but as for many algorithms \cite{simchowitz_simulator_2017, gabillon_best_2012, auer_pareto_2016} we do not control what happens on $\cE^\complement$. Therefore, the goal here is to upper-bound $\bE(\tau)$ instead of $\bE(\ind\{\cE\}\tau)$ which we did in \autoref{thm:sampcompl}. To adapt the strategy employed in \cite{kalyanakrishnan_pac_2012}, we use similar confidence bonuses, hence we define for any arm $i$, 
\begin{equation}
    \label{eq:beta-single}
    \beta_i(t) = \sqrt{\frac{2}{T_i(t)}\log\left(\frac{5KDt^4}{2\delta}\right)},
\end{equation}
and for any $i,j\in\bA$, $\beta_{i,j}(t) = \beta_i(t) + \beta_j(t)$. Recalling the definition of $\cE$ and $\cE_t$ introduced in section 3.1, 
\begin{eqnarray*}
    \cE_t := \bigcap_{i=1}^K \bigcap_{j\neq i}\bigcap_{d=1}^D   \{L^d_{i,j}(t, \delta) \leq \mu_i^d - \mu_j^d \leq U^d_{i,j}(t, \delta)\}, \ \text{ and } \ \cE = \bigcap_{t =1}^{\infty} \cE_{t},
\end{eqnarray*}
the lemma hereafter shows that with the choice of $\beta_i$'s in \eqref{eq:beta-single} and for $1$-subgaussian marginals, $\bP(\cE) \geq 1-\delta$. 
\begin{lemma}
\label{lem:correctness-single-beta}
   It holds that $\bP(\cE) \geq 1 - \delta.$
\end{lemma}
\begin{proof}
    Letting $$\tilde \cE_t := \bigcap_{i=1}^K\bigcap_{d=1}^D \lvert \muh_i^d(t) - \mu_i^d\lvert \leq \beta_i(t), $$
    we have $\tilde \cE_t \subset \cE$. Indeed, on $\tilde \cE_t$, for any $i,j\in \bA$ and $d\leq D$, $$ \muh_i^d(t) - \muh_j^d(t) - \beta_i(t) - \beta_j(t) \leq \mu_i^d - \mu_j^d \leq \muh_i^d(t) - \muh_j^d(t) + \beta_i(t) + \beta_j(t).$$
Setting $\beta_{i,j}(t) = \beta_i(t) + \beta_j(t)$ yields  $\tilde \cE_t \subset \cE_t$ so 
\begin{equation}
 \bP(\cE^\complement
) \leq \sum_{t=1}^\infty \bP(\cE_t^\complement) \leq \sum_{t=1}^\infty \bP(\tilde \cE_t^\complement).  
\end{equation}
Applying Hoeffding's to the $1$-subgaussian marginals yields 
\begin{eqnarray}
    \bP(\tilde \cE_t^\complement) &\leq& \sum_{i=1}^K \sum_{d=1}^D  \bP(\lvert\muh_i^d(t) - \mu_i^d\lvert > \beta_i(t)), \\
    &\leq& \sum_{i=1}^K \sum_{d=1}^D \sum_{s=1}^t \bP(\lvert\muh_{i, s} - \mu_i^d\lvert > \beta^{t, s}) \quad \text{ where } \beta^{t, s} = \sqrt{\frac{2}{s}\log\left(\frac{5KDt^4}{2\delta}\right)},\\
    \label{eq:ub-proba-cE-tilde}
    &\leq& \sum_{i=1}^K \sum_{d=1}^D \sum_{s=1}^t \frac{4\delta}{5KDt^4}, \\ &=& \frac{4\delta}{5t^3}.
\end{eqnarray}
Finally, 
\begin{eqnarray}
 \bP(\cE^\complement
) &\leq&  \sum_{t=1}^\infty \bP(\tilde \cE_t^\complement), \\
&\leq& \frac{4\delta}{5} \sum_{t=1}^\infty \frac{1}{t^3},\\
&\leq& \delta. 
\end{eqnarray}
\end{proof}
We can now state the following theorem. 
\begin{theorem}
Let $\eps_1 \geq 0, k\leq K$ and $\nu$ a bandit with $1$-subgaussian marginals. 
\algname run with the $\beta_i'$s of \eqref{eq:beta-single} and associated to the stopping time $\tau_{\eps_1}^k$ outputs a valid set and the expected sample complexity is upper bounded as follows :  
$$ \bE_{\nu}(\tau_\delta) \leq \inf_{\gamma \in (0,1)} \left\{\frac{128\sqrt e}{1-\gamma} \log\left( \frac{128(5KD/(4\delta)^{1/4})\sigma^2 H}{1-\gamma}\right)  + \frac{2\pi^2}{15} \frac{1 - \gamma}{\gamma^3}  \right\} + 1.$$
\end{theorem}
% TODO ref de la proof (kalyanakrishnan ? )
% TODO utiliser gamma = 1/2 comme dans LUCB ?
\begin{proof}[Proof of \autoref{thm:sampcompl}]
The correctness follows from \autoref{lem:correctness-generic} and \autoref{lem:correctness-single-beta}. It remains to upper-bound $\bE(\tau_{\eps_1}^k)$. This proof technique has been already employed in \cite{kalyanakrishnan_pac_2012, kaufmann_information_2013, jun_anytime_2016}.
Let $0<\gamma< 1$, and for any $n\geq 1$, let 
\begin{eqnarray}
\cE(n) &=& \bigcap_{t\in [\gamma n, n]} \cE_t.
\end{eqnarray}
We have 
\begin{eqnarray*}
    \cE(n) \cap \{ \tau_{\eps_1}^k > n\} \tm{ holds } &\impl& \ind\{\cE(n)\}\sum_{t=1}^n \ind\{\tau_{\eps_1}^k > t\} = \sum_{t=1}^n \ind\{\{\tau_{\eps_1}^k> t\}\cap \cE(n)\} = n .
\end{eqnarray*}
Then, upper-bounding the RHS yields 
\begin{eqnarray}
\label{eq:exp_sampl_eq1}
\sum_{t=1}^n \ind\{\{\tau_{\eps_1}^k > t\}\cap \cE(n)\} &\leq& \gamma n +   \sum_{t=\gamma n}^n \ind\{\{\tau_{\eps_1}^k > t\}\cap \cE(n)\}, \\&\leq& 
\gamma n + \sum_{t=\gamma n}^n \ind\{ (\tau_{\eps_1}^k > n)\land \cE_t \}. 
\end{eqnarray}
From \autoref{lem:samplold}, \autoref{lem:sampl-complex-eps} and \autoref{lem:samplwm}, we have that for any $t\in [\gamma n, n]$, 
$$ \{\tau_{\eps_1}^k > t\}\cap \cE_t \impl \max(\Delta_{a_t}, \eps_1, \omega_k) \leq 2\beta_{a_t, a_t}(t), $$ with $\beta_{a_t, a_t} = 2\beta_{a_t}(t)$. Therefore, 
%and from the proof of \autoref{thm:sampcompl}, 
%$$ \{\tau_\delta > t\}\cap \cE_t \impl \Delta_{k_t} \leq 4\beta_{k_t}(t), $$
%where $k_t$ is the least sampled arm among $b_t$ and $c_t$. 
using this result back in \eqref{eq:exp_sampl_eq1} and letting $C := ({5KD}/{(2\delta)})^{1/4}$, $\tilde \Delta_a := \max(\Delta_a, \eps_1, \omega_k)$ yields 
\begin{eqnarray}
  \sum_{t=1}^n \ind\{\{\tau_{\eps_1}^k > t\}\cap \cE(n)\} %&\leq& \gamma n +   \sum_{t=\gamma n}^n \ind\{\{\tau_\delta > t\}\cap \cE(n)\},   \\
  %&\leq& \gamma n + \sum_{t=\gamma n}^n \ind\{ (\tau_\delta > t)\land \cE_t \} \\
  &\leq& \gamma n + \sum_{t=\gamma n}^n\ind\{ \tilde \Delta_{a_t} \leq 4\beta_{a_t}(t) \}\\&\leq& \gamma n + \sum_{t=\gamma n}^n\sum_{a=1}^K\ind\{ (a_t = a) \land \tilde \Delta_a \leq 4\beta_{a}(t) \}, \\
  &\leq& \gamma n + \sum_{a=1}^K\sum_{t=\gamma n}^n \ind\{(a_t = a) \land (T_{a}(t) \leq \frac{128}{\Delta_a^2}\log(C t))\}\\
  &\leq& \gamma n + \sum_{a=1}^K \sum_{t=\gamma n}^n \ind\{(a_t = a) \land (T_{a}(t) \leq \frac{128}{\Delta_a^2}\log(Cn))\} \\
  &\leq& \gamma n + \sum_{a=1}^K \frac{128}{\Delta_a^2}\log(C n)\\
  &\leq& \gamma n + 128 H \log(C n), 
\end{eqnarray}
then, choosing  $n$  such that 
$$\gamma n + 128 H \log(C n) < n, $$
that is  
$$ n > T^\star := \inf \left\{ s\in \bN^\star : \frac{128 H \log(Cs)}{s}< 1 - \gamma \right\},$$
would yield 
\begin{equation}
    \sum_{t=1}^{n} \ind\{\{\tau_{\eps_1}^k > t\}\cap \cE(n)\} < n, 
\end{equation}
therefore, for any $n>T^\star$, $$\cE(n) \cap \{ \tau_{\eps_1}^k > n\} = \emptyset,$$ which means $$\{\tau_{\eps_1}^k > n\} \subset \cE(n)^\complement.$$  
Thus, 
\begin{eqnarray}
 \bE_{\nu}(\tau_{\eps_1}^k)  &=&    \bE_{\nu}\left(\tau_{\eps_1}^k \ind\{\tau_{\eps_1}^k \leq T^\star\} + \tau_{\eps_1}^k \ind\{\tau_{\eps_1}^k > T^\star \} \right)\\
 &\leq& T^\star  + \bE_{\nu}(\tau_{\eps_1}^k \ind\{\tau_{\eps_1}^k> T^\star \}\\
 &\leq& T^\star  + \sum_{n=T^\star + 1}^\infty \bP_\nu(\tau_{\eps_1}^k > n)\\
 &\leq& T^\star  + \sum_{n=T^\star + 1}^\infty \bP_\nu(\cE(n)^\complement), 
\end{eqnarray}
using \eqref{eq:ub-proba-cE-tilde} and union bound yields, 

\begin{eqnarray}
 \bP(\cE(n)^\complement) &\leq&  \sum_{t=\gamma n}^n \frac{4\delta}{5t^3},\\&\leq& \frac{4\delta}{5} \frac{(1 - \gamma)n}{\gamma^3n^3},  \\
 &=& \frac{4\delta}{5} \frac{1 - \gamma}{\gamma^3}\frac{1}{n^2}.
\end{eqnarray}
Then, 
\begin{eqnarray}
   \bE_{\nu}(\tau_{\eps_1}^k)  &\leq&     T^\star  + \frac{4\delta}{5} \frac{1 - \gamma}{\gamma^3} \frac{\pi^2}{6}\\
   &\leq& T^\star +  \frac{2\pi^2}{15} \frac{1 - \gamma}{\gamma^3}.
\end{eqnarray}
Upper-bounding $T^\star$ will conclude the proof. 
\begin{lemma} 
\label{lem:bound_T_star}
It holds that
    $$T^\star -1 \leq  \frac{1}{c_\delta} \exp\left(-W_{-1}\left( -\frac{1-\gamma}{128c_\delta H} \right)\right) \leq \frac{128\sqrt e H}{1-\gamma}\log\left( \frac{128c_\delta H }{1-\gamma}\right).$$
\end{lemma}
Finally, 
\begin{eqnarray}
 \bE_{\nu}(\tau_\delta) &\leq& \frac{128\sqrt e H}{1-\gamma} \log\left( \frac{128(5KD/(2\delta))^{1/4} H}{1-\gamma}\right)  + \frac{2\pi^2}{15} \frac{1 - \gamma}{\gamma^3} + 1,   \\
 &\leq&  
\frac{53 H}{1-\gamma}\log\left( \frac{5KD}{2\delta}\right) + 
\frac{128\sqrt e H}{1-\gamma} \log\left( \frac{128H}{1-\gamma}\right) + \frac{2\pi^2}{15} \frac{1 - \gamma}{\gamma^3} + 1, 
\end{eqnarray}
% \begin{equation}
%    \bE_{\nu}(\tau_\delta) \leq \frac{128\sqrt e H}{1-\gamma} \log\left( \frac{128(5KD/(4\delta)^{1/4}) H}{1-\gamma}\right)  + \frac{2\pi^2}{15} \frac{1 - \gamma}{\gamma^3} + 1,
% \end{equation}
which achieves the proof. 
\begin{remark}
The same technique could be applied to upper-bound $\bE_\nu(\tau_{\eps_1, \eps_2})$. 
\end{remark}
% \begin{remark}
% For $D=1$ and using $(5K/4) \leq H$, which is likely to be the case for any non-trivial instance, $\gamma = 1/2, \sigma = 1/2$, we have 
% $\bE_{\nu}(\tau_\delta) \leq 132H\log(\frac{28H}{\delta^{1/5}}) +7$. 
% \end{remark}
%% A deplacer
    \begin{proof}[Proof of \autoref{lem:bound_T_star}]
        We have 
         \begin{eqnarray}
         \label{eq:eq_bound_T_star1}
             128 H\frac{\log(c_\delta s)}{s} < 1-\gamma  &\equi& \frac{\log(c_\delta s)}{ s} < \frac{1 - \gamma }{128H} 
         \end{eqnarray}
         then, using \autoref{lem:ineq_log} yields 
         \begin{eqnarray*}
             \eqref{eq:eq_bound_T_star1} &\impl& \begin{cases}
                 s > 0 & \tm{ if } \frac{1-\gamma}{128H} <c_\delta / e \\
                 0<s\leq \frac{1}{c_\delta} \; \tm{or}\; s \geq N^\star & \tm{ else, }
             \end{cases}
         \end{eqnarray*}
         with
         $$ N^\star = \frac{1}{c_\delta} \exp\left(-W_{-1}\left( -\frac{1-\gamma}{128c_\delta H } \right)\right).$$
         Therefore, 
         $$ T^\star = \inf\{s \in \bN^\star : 128H\frac{\log(c_\delta s)}{s} < 1-\gamma\} \leq    \begin{cases}
            1  & \tm{ if }  \frac{1-\gamma}{128H} <c_\delta / e\\
            \ceil{N^\star} & \tm{ else.}
         \end{cases} $$
         Using \autoref{lem:bound_W_1}, to upper bound $N^\star$ yields 
         \begin{equation}
             T^\star - 1 \leq \frac{128\sqrt{e} H}{1-\gamma}\log_+\left( \frac{128c_\delta H }{1-\gamma}\right),
         \end{equation}
         where $\log_+(x) = \max(0, \log(x))$. 
    \end{proof}
% \begin{lemma}
%     $\bP(\cE(n)^\complement)\leq \frac{4}{5\delta} \frac{1}{n^2}$.
%     \begin{proof}
%         \bP()
%     \end{proof}
% \end{lemma}
\end{proof}
\section{Technical Lemmas}
\label{sec:tech_lemmas}
\begin{lemma}
\label{lem:ineq_log}
    Let $a, b>0$. If $b < a/e$ then 
    $$ \frac{\log(ax)}{x} < b \impl  0<x \leq \frac1a \;\tm{or}\;x \geq \frac{1}{a}\exp\left(-W_{-1}\left(-\frac{b}{a}\right)\right).$$
Moreover, if $b\geq a/e$, then for any $x>0$, $\log(ax)/x \leq b$. 
\end{lemma}
\begin{proof}
    We have 
    \begin{eqnarray*}
        \frac{\log(ax)}{x} < b &\impl&  -\frac{1}{ax} \log\left(\frac{1}{ax}\right) < \frac ba \\&\impl& y \log(y) > - \frac{b}{a}, \quad y = \frac{1}{ax} \\
        &\impl& \frac{1}{ax} \geq  1 \; \tm{or} \; -\frac{b}{a}<y\log(y) < 0 
    \end{eqnarray*}
since $-b/a>-1/e$ and the negative branch $W_{-1}$ of the Lambert function is decreasing on $[-1/e, 0]$, 
\begin{eqnarray*}
 \frac{\log(ax)}{x} < b &\impl& 0<x \leq \frac{1}{a}  \; \tm{or} \; W_{-1}(y\log(y)) \leq W_{-1}(-b/a) \\
 &\impl& 0<x \leq \frac{1}{a}  \; \tm{or} \; \log(y) \leq W_{-1}(-b/a) \\
  &\impl& 0<x \leq \frac{1}{a}  \; \tm{or} \; ax \geq \exp(-W_{-1}(-b/a))\\
  &\impl& 0<x \leq \frac{1}{a}  \; \tm{or} \; x \geq \frac1a\exp(-W_{-1}(-b/a)). 
\end{eqnarray*}
Proving the second part of the lemma just follows from $\log(x) \leq x/e$. 
\end{proof}
%TODO lemma ref
The following lemma is taken from \cite{jourdan_top_2022}
\begin{lemma}[\cite{jourdan_top_2022}]
\label{lem:lambert_dom}
    For any $x \in [0, -e^{-1}]$, 
    \[  -\log(-x) + \log(-\log(-x)) \leq - W_{-1}(x) \leq -\log(-x) + \log(-\log(-x)) + \min\left\{ \frac12, \frac{1}{\sqrt{-x\log(-x)}}\right\} \]
\end{lemma}

\begin{corollary}
\label{lem:bound_W_1}
    Let $0<a<1/e$. It holds that 
    $$ \exp(-W_{-1}(-a)) \leq \frac{e^{1/2}}{a}\log\left(\frac{1}{a}\right).$$
\end{corollary}
\begin{proof}
    Using \autoref{lem:lambert_dom} yields, 
    $$- W_{-1}(-a) \leq -\log(a) + \log(-\log(a)) + \frac12,$$
    and taking $\exp$ on both sides gives the result.
\end{proof}
% \begin{lemma}{\cite{kaufmann_complexity_2014}}
%     Let $X_1, X_2, \dots$ be \iid centered $\sigma$-sub-gaussian random variables and $\delta \in (0,1)$. With probability at least $1-\delta$, 
%     \[ \forall t \geq 1, \; \lvert t^{-1}\sum_{s=1}^t X_s\lvert   \leq \sigma\sqrt{\frac{2 \log(1/\delta) + 6\log\log(1/\delta) + 3\log\log(et)}{t}} =: f(t, \sigma). \]
% \end{lemma}

\begin{lemma}{\cite{kaufmann_mixture_2021}}
Let $X, Y$ be centered $\sigma-$subgaussian random variables and $\delta \in (0,1)$. 
Let $X, X_1, X_2, \dots$ be \iid  random variables and $Y, Y_1, Y_2, \dots$ be \iid random variables. 
With probability at least $1-\delta$, 
    \[ \forall p, q \geq 1, \; \lvert p^{-1}\sum_{s=1}^p X_s  - q^{-1}\sum_{s=1}^q Y_s \lvert\leq 2\sqrt{\left(C^g\left(\frac{\log({1}/{\delta})}{2}\right) + \log\log(e^4 p) + \log\log(e^4q)\right) \left(\frac{1}{p} + \frac{1}{q}\right)} \]
where $C^g(x) \approx x + \log(x)$
\end{lemma}

\begin{lemma}
\label{lem:bound_part_tps}
    Let $\Delta^2>0$. Then, for $t\geq 2$, 
    $$ t \geq \frac{1}{\Delta^2}\log\left(2\log\left(\frac{3e^2}{2\Delta^2}\right)\right) \impl \frac{\log\log\left(e^4t\right)}{t} < \Delta^2.$$
\end{lemma}
   \begin{proof}
    We note that if $\Delta^2 \geq \frac{e}{3}$, then the result follows trivially since it can be easily checked that for $t\geq 2$,
    $$ \log\log(e^4t) \leq \frac{e}{3}t.$$
    Therefore, in the sequel, we assume $\Delta^2 < e/3$. 
        Let $$t_\Delta := \frac{1}{\Delta^2}\log\left(2\log\left(\frac{3e^2}{2\Delta^2}\right)\right),$$ and 
        $$ g(t) = t - \frac{1}{\Delta^2}{\log(\log(e^4t))}.$$
     Then, 
     $$g'(t) = 1 - \frac{1}{\Delta^2 t \log(e^4t)},$$
     and $g'(t) \geq 0$ for $t$ such that $\Delta^2 t\log(e^4t)\geq 1$. Using the Lambert function $W_0$, which is increasing on $[0, \infty)$,
        \begin{eqnarray}
             \Delta^2 t\log(e^4t) \geq 1 &\equi& e^4t\log(e^4t) \geq \frac{e^4}{\Delta^2} \\ &\equi& \log(e^4t) \geq W_0\left(\frac{e^4}{\Delta^2}\right)\\
             &\equi& t\geq t^0:=\frac1{e^4} \exp\left(W_0\left(\frac{e^4}{\Delta^2}\right)\right)
        \end{eqnarray}   
    and by definition of $W_0$, we have $$ W_0(x)\exp(W_0(x)) = x,$$ so 
    $$ \exp\left(W_0\left(\frac{e^4}{\Delta^2}\right)\right) = \frac{e^4}{\Delta^2} \frac{1}{W_0(e^4\Delta^{-2})}, $$
and therefore, 
$$
t^0 = \frac{1}{\Delta^2} \frac{1}{W_0(e^4\Delta^{-2})}.
$$
We will show that $t_\Delta > t^0$. Indeed, since $W_0$ is increasing, %and $\frac{1}{\Delta^2} > 3/e$, 
    \begin{eqnarray*}
        \frac{1}{\Delta^2} > 3/e &\impl& W_0\left(\frac{e^4}{\Delta^2}\right) \geq W_0(3e^3) = 3 \\&\impl& 
        \frac{1}{\Delta^2} \frac{1}{W_0(e^4\Delta^{-2})} \leq \frac{1}{3} \frac{1}{\Delta^2} ,
    \end{eqnarray*}
    that is 
    \begin{equation}
\label{eq:upper-bound-t0}
t^0 \leq  \frac13 \frac{1}{\Delta^2} . 
    \end{equation}
On the other side, 
\begin{eqnarray*}
    \frac{1}{\Delta^2} > 3/e &\impl& \log\left(2\log\left(\frac{3e^2}{2\Delta^2}\right)\right) > \log(2\log(9e/2)) \\
    &\impl& t_\Delta \geq \frac{1}{\Delta^2}\log(2\log(9e/2))> \frac13 \frac1{\Delta^2}
\end{eqnarray*}
Therefore, \begin{equation*}
   t^0 \leq \frac13\frac{1}{\Delta^2} <\frac{\log(2\log(9e/2))}{\Delta^2} \leq t_\Delta. 
\end{equation*}
 Thus, we have shown that $t^0 \leq t_\Delta$  and for any $t\geq t_\Delta$, $g'(t) \geq 0$  so 
 \begin{equation}
 \forall t \geq t_\Delta, \; g(t) \geq g(t_\Delta).    
 \end{equation}
 Showing that  $g(t_\Delta) > 0$, will conclude the proof. 
Letting $a = 3e^2/2$, we have 
 \begin{eqnarray}
 g(t_\Delta) > 0   &\equi& \frac{1}{\Delta^2}\log(2\log(a/\Delta^2)) - \frac{1}{\Delta^2}\log(\log(e^4t_\Delta)) > 0 \\
  &\equi& \log(2\log(a/\Delta^2)) - \log(\log(e^4t_\Delta)) > 0 \\
   &\equi& 2\log(a/\Delta^2) - \log(e^4t_\Delta) > 0 \\
   &\equi& \log(a/\Delta^2) - \log(e^4t_\Delta\Delta^2  /a) >0 \\
    &\equi& \frac{a}{\Delta^2} - \frac{e^4}{a}{\Delta^2} t_\Delta > 0 \\
    \label{eq:sign_g}
    &\equi& \frac{a}{\Delta^2} - \frac{e^4}{a}\log(2\log(a/\Delta^2))> 0,
\end{eqnarray}
then,  observing that for $x\geq 12$, 
$$ \log(2\log(x)) \leq \frac{x}{e^2},$$
and since $$ a/\Delta^{2}  > (3e^2/2) \times (3/e) > 12,$$
we have 
\begin{equation}
\label{eq:bound-log-log}
    \log(2\log(a/\Delta^2)) \leq \frac1{e^2} \frac{a}{\Delta^2}
\end{equation}
%since $\log(x)\leq x/e$, 
%$$ e\log(2\log(1/\Delta^2)) \leq  \frac{2}{e\Delta^2},$$
so, using \eqref{eq:bound-log-log} yields that the LHS of \eqref{eq:sign_g} is larger than 
$$\frac{3}{2}e^2 \frac1{\Delta^2} - e^2 \frac1{\Delta^2}, $$
which is always positive. 
Therefore, \begin{equation*}
    \forall t \geq t_\Delta,\; g(t_\Delta) > 0 , 
\end{equation*}
that is 
\begin{equation}
    \forall t \geq t_\Delta, \; \frac{\log\log(e^4t)}{t} < \Delta^2.
\end{equation}
    \end{proof}
% Therefore, $g'(t)\geq 0$, for any $t\geq b^{-1}\exp(W_0(\Delta^{-2}))=:t^0$. In the sequel assume $t_\Delta \geq t^0$. So, for $t\geq t_\Delta$, $g(t) \geq g(t_\Delta)$ and 
% \begin{eqnarray}
%  g(t_\Delta) > 0   &\equi& \frac{1}{\Delta^2}\log(2a\log(ab/\Delta^2) - \frac{1}{\Delta^2}\log(a\log(bt_\Delta)) > 0 \\
%   &\equi& \log(2a\log(ab/\Delta^2) - \log(a\log(bt_\Delta)) > 0 \\
%    &\equi& 2\log(ab/\Delta^2) - \log(bt_\Delta) > 0 \\
%    &\equi& \log(ab/\Delta^2) - \log(\Delta^2 t_\Delta/a) >0 \\
%     &\equi& \frac{ab}{\Delta^2} - \frac{\Delta^2}{a} t_\Delta > 0 \\
%     %\label{eq:sign_g}
%     &\equi& \frac{ab}{\Delta^2} - \frac{1}{a}\log(2a\log(ab/\Delta^2))> 0,
% \end{eqnarray}
% then, since 
% $$ - \frac{1}{a}\log(2a\log(ab/\Delta^2)) \geq - \frac{2ab}{e^2\Delta^2},$$
% where we have used that $\log(x) \leq x/e$, it comes
% $$ \frac{ab}{\Delta^2} - \frac{1}{a}\log(2a\log(ab/\Delta^2)) \geq  \frac{ab}{\Delta^2}(1 - \frac{2}{e^2}) >0.$$ Therefore, the RHS of \eqref{eq:sign_g} is positive, hence $g(t_\Delta)>0$ and for $t\geq t_\Delta,$
% $g(t)>0$, that is 
% $$ f(t) \leq \Delta.$$
% Now, it remains to show that $t_{\Delta}\geq t^0$. We have 
% \begin{eqnarray*}
%    0<t_{\Delta}<  t^0 &\impl&  t_\Delta \log(t_\Delta) < t^0\log(t^0) \\
%   &\impl& t_\Delta \log(t_\Delta) < \Delta^{-2} \\
%   &\impl& \frac{1}{\Delta^2}\log(2a\log(ab/\Delta^2)) \log(t_\Delta) < \frac{1}{\Delta^2} \\
%   &\impl& \log(2a\log(ab/\Delta^2)) \times \log({\Delta^{-2}}\log(2a\log(ab/\Delta^2))) < 1 \\
%   &\impl& x\log(\Delta^{-2}x) < 1 \qquad \tm{ where } x = \log(2a\log(ab/\Delta^2))
% \end{eqnarray*}
\begin{lemma}
\label{lem:bound_inv_beta}
   Let $\delta \in (0, 1), \Delta> 0$ and $c>0$. Let $f : t \mapsto \sqrt{ \frac{g(\delta) + c\log\log(e^4t)}{t}}$
    where $g$ is a non-negative function. Then, for any $\alpha \in (0,1)$ and $t\geq 2$, 
    \begin{equation}
        t \geq \frac{1}{\Delta^2} \left( \frac{1}{\alpha} g(\delta) + \frac{c}{1-\alpha}\log_+\left(2\log\left(\frac{c}{(1-\alpha)\Delta^2}\right)\right)\right) \impl f(t) < \Delta. 
    \end{equation}
    \end{lemma}
        \begin{proof}
       Letting $t\geq 2$, we have 
        \begin{equation}
\label{eq:eq_bound_inv_beta_1}
            t \geq t_1:= \frac1\alpha\frac{1}{\Delta^2} g(\delta) \impl \frac{g(\delta)}{t} \leq \alpha \Delta^2. 
        \end{equation}
        Furthermore, using \autoref{lem:bound_part_tps} yields 
        \begin{equation}
\label{eq:eq_bound_inv_beta_2}
            t \geq t_2:= \frac{c}{(1- \alpha)\Delta^2} \log_+\left(2\log\left(\frac{3e^2}{2(1-\alpha)\Delta^2}\right)\right) \impl \frac{\log\log(e^4t)}{t} \leq (1- \alpha)\Delta^2/c.
        \end{equation}
        Combining \eqref{eq:eq_bound_inv_beta_1} and \eqref{eq:eq_bound_inv_beta_2} yields for $t\geq 2$,
        \begin{eqnarray*}
            t \geq \max(t_1, t_2) \impl f(t)^2 < \Delta^2, 
        \end{eqnarray*}
        so \begin{equation}
            t \geq t_1 + t_2\geq \max(t_1, t_2) \impl f(t) < \Delta. 
        \end{equation}
    \end{proof}

\begin{lemma}
\label{lem:bound_inv_beta_ek}
Let $\sigma, \Delta > 0$. Let 
 \[ f(t) := 4\sqrt{\frac{2 C^g(\log(1/\delta)/2) + 4\log\log(e^4t)}{t}}.\]
 Then 
$$ \inf\{n\geq 2 : f(n) < \Delta \} \leq \frac{88}{\Delta^2}\log\left(\frac{4}{\delta}\log\left(\frac{12e}{\Delta^2}\right)\right).$$
\end{lemma}
\begin{proof}
We have 
\begin{eqnarray*}
  f(t) = \sqrt{\frac{32 C^g(\log(1/\delta)/2) + 64\log\log(e^4t)}{t}}.%  \sqrt{\frac{g(\delta) + \log\log(et)}{t}} < \frac{\Delta}{\sigma\sqrt{3}},< \Delta &\equi&  
\end{eqnarray*}
%further using $C^g(x) \approx x + \log(x)$ \cite{kaufmann_mixture_2021} yields 
%$$ 32 C^g(\log(1/\delta)/2) \approx 16\log(1/\delta) + 32\log$$
%where 
%$$ g(\delta) := (2/3)\log(1/\delta) + 2\log\log(1/\delta).$$
Therefore, letting 
$$ g(\delta):= 32 C^g(\log(1/\delta)/2) \quad \text{ and } \quad  c= 64$$ and further using \autoref{lem:bound_inv_beta} yields for any $\alpha \in (0, 1)$ and $t\geq 2$, 
$$ t\geq t_{\alpha} \impl f(t) < {\Delta},$$
where 
$$ t_{\alpha} := \frac{1}{\Delta^2} \left(\frac{32}{\alpha}C^g(\log(1/\delta)/2) + \frac{64}{1-\alpha}\log\left(2\log(96e^2(1-\alpha)^{-1}\Delta^{-2})\right)\right).$$
   Since $C^g(x)\approx x + \log(x)$ \cite{kaufmann_mixture_2021},  and $\log(x) \leq x/e$ we have 
   $$ \Delta^2 t_{\alpha} \leq \left({16}  + \frac{16}{e}\right)\frac{1}{\alpha}\log(1/\delta) +  \frac{64}{1-\alpha}\log(2\log(96e^2(1-\alpha)^{-1}\Delta^{-2})).$$
Taking $\alpha = \alpha^\star$ such that $$\left({16}  + \frac{16}{e}\right)\frac{1}{\alpha^\star} = \frac{64}{1-\alpha^\star},$$
that is setting \begin{equation}
    \alpha^\star = \frac{1+e}{1+5e}, 
\end{equation}
yields
$$\Delta^2 t_{\alpha^\star} \leq \frac{64}{1 - \alpha^\star}\log\left( \frac2\delta \log\left( \frac{96e^2}{(1-\alpha^\star) \Delta^2}\right)\right).$$
By numerical evaluation, 
$$ \frac{64}{1 - \alpha^\star}  \approx 86 < 88 \quad \text{ and } \quad \frac{96}{1-\alpha^\star} \approx 130 <  12^2,$$
so 
\begin{equation}
\Delta^2 t_{\alpha^\star} < 88\log\left( \frac4\delta \log\left( \frac{12e}{\Delta^2}\right)\right). 
\end{equation}
Therefore, 
putting these results together, for $t\geq 2$
$$t\geq  t_{\star} := \frac{88}{\Delta^2}\log\left( \frac4\delta \log\left( \frac{12e}{\Delta^2}\right)\right) \impl f(t) < \Delta$$ which yields
\begin{equation}
\inf\{n\geq 2: f(n) < \Delta \} \leq \max(2, t_\star).    
\end{equation}
\end{proof}
\section{Implementation and Additional Experiments}
\label{sec:impl_exp}
\subsection{Implementation}
\label{subsec:implementation}
In this section, we give additional details about the experiments and additional results.
\paragraph{Setup :} We have implemented the algorithms mainly in \texttt{C++17} interfaced with \texttt{python} through \texttt{cython}. The experiments are run on an ARM64 8GB/8 core/256GB disk storage computer. 
For the function $C^g$ we use the approximation $C^g(x) \approx x + \log(x)$  which is usually admitted \cite{kaufmann_mixture_2021}.  
For the experiments on real-world scenario we generate a certain number of seeds (usually 2000) and for we use  a different seed for each run on the same bandit.  This procedure is repeated for every experiment where we report the average sample complexity on the same bandit. To assess the robustness of our algorithm, the experiments on the synthetic dataset consists in randomly uniformly sampling some bandit means for each configuration. For each sampled bandit, the algorithms to compare are run once on the same instance and we note their empirical sample complexity. Finally, we report the average sample complexity across all the bandits of the same configuration.  
\subsection{Data processing}
\label{subsec:data_processing}
\paragraph{Dataset: } The dataset is extracted from \cite{munro_safety_2021} and some processing steps are applied to compute the covariance matrix of the distribution. First, as observed in \cite{munro_safety_2021}, the 3 immunogenicity indicators extracted are weakly correlated, therefore, we assume the covariance matrix to be diagonal. To compute the variance of the marginals, we use the log-normal assumption as assumed for the data reported in \cite{munro_safety_2021}. 
Using this log-normal assumption 
the authors have provided for each arm and each indicator: the geometrical mean, the sample size and a $95\%$ confidence interval on the geometrical mean based on \emph{central limit theorem}. We use these information and to compute the sample variance of each immunogenicity indicator. We compute the arithmetic average of the $\log$ outcomes which are obtained by taking the $\log$ (base $e$) of the geometrical empirical mean. This represents by assumption the mean of a Gaussian distribution. We will therefore use these values to simulate a Gaussian distribution. The variance are obtained by the \emph{central limit theorem} and we report the pooled variance of each indicator in \autoref{tab:pooled_var}. In \autoref{tab:arith_mean} we report the average outcomes after the processing. There are 20 arms classified into two groups. Each three/four-letters acronym denote a vaccine candidate. Prime BNT/BNT corresponds to giving BNT as first and second dose and similarly for Prime ChAd/ChAd. For example ChAd in the group Prime BNT/BNT means to give BNT as first and second dose and ChAd as third dose (booster). 
\begin{table}[H]
\caption{Table of the empirical arithmetic mean of the log-transformed immune response for three immunogenicity indicators. Each acronym corresponds to a vaccine (or arm). There are two groups of arms corresponding to the first 2 doses: one with prime BNT/BNT (BNT as first and second dose) and the second with prime ChAd/ChAd (ChAd as first and second dose).}
\begin{center}
\begin{tabular}{|c|c|c|c|c|}
\hline 
\hline 
\multirow{2}{*}{Group} & \multirow{2}{*}{Arm}  &\multicolumn{3}{c|}{Immune response}\\
 &  & Anti-spike IgG &  $\text{NT}_{50}$ &  cellular response\\\hline 
    \multirow{10}{*}{Prime BNT/BNT}&ChAd     &                      9.50 &                                       6.86 &                                 4.56 \\
&NVX      &                      9.29 &                                       6.64 &                                 4.04 \\
&NVX Half &                      9.05 &                                       6.41 &                                 3.56 \\
&BNT      &                     10.21 &                                       7.49 &                                 4.43 \\
&BNT Half &                     10.05 &                                       7.20 &                                 4.36 \\
&VLA      &                      8.34 &                                       5.67 &                                 3.51 \\
&VLA Half &                      8.22 &                                       5.46 &                                 3.64 \\
&Ad26     &                      9.75 &                                       7.27 &                                 4.71 \\
&m1273    &                     10.43 &                                       7.61 &                                 4.72 \\
&CVn      &                      8.94 &                                       6.19 &                                 3.84 \\
\hline
 \multirow{10}{*}{Prime ChAd/ChAd}&ChAd     &                      7.81 &                                       5.26 &                                 3.97 \\
&NVX      &                      8.85 &                                       6.59 &                                 4.73 \\
&NVX Half &                      8.44 &                                       6.15 &                                 4.59 \\
&BNT      &                      9.93 &                                       7.39 &                                 4.75 \\
&BNT Half &                      8.71 &                                       7.20 &                                 4.91 \\
&VLA      &                      7.51 &                                       5.31 &                                 3.96 \\
&VLA Half &                      7.27 &                                       4.99 &                                 4.02 \\
&Ad26     &                      8.62 &                                       6.33 &                                 4.66 \\
&m1273    &                     10.35 &                                       7.77 &                                 5.00 \\
&CVn      &                      8.29 &                                       5.92 &                                 3.87 \\
\hline
\end{tabular}
\end{center}
\label{tab:arith_mean}
\end{table}
\begin{table}[ht]
\caption{Pooled variance of each group.}
\begin{center}
\begin{tabular}{|c|c|c|c|}
\hline 
\hline 
\multirow{2}{*}{Group} & \multicolumn{3}{c|}{Immune response}\\
 & Anti-spike IgG &  $\text{NT}_{50}$ &  cellular response\\\hline 
     Prime BNT/BNT&  0.61& 0.78& 1.69\\
         Prime ChAd/ChAd & 0.78 & 0.86 & 1.39\\\hline
\end{tabular}
\end{center}
\label{tab:pooled_var}
\end{table}
\subsection{Additional experiments}
\label{subsec:additional_experiments}
\subsubsection{Additional experiments for $\eps_1$-APE-$k$}
In this section we show that for some instances our algorithm can require up to 3 times less samples compared to \algauername. This is due to the strategy of \algauername which samples continue sampling arms identified as optimal until there are shown not to dominate an arm in the active set. For example on \autoref{fig:config-avantage-APE}, the optimal arm 2 is "easy" to identify as such. However, since it it slightly dominate the sub-optimal arm 1, \algauername will continue sampling arm 2 until arm 1 is removed from the active set ( likely this will happen when the algorithm "sees" that arm 1 is dominated by arm 3).  We would expect our adaptive sampling rule to avoid this behaviour. \autoref{fig:appx-new-instance-ape-k-sc} shows that APE takes nearly half the average sample complexity of \algauername on this instance. In particular, \autoref{tab:average-pull-ratio} shows the average number of pulls taken  by \algauername divided by the average number of pulls taken by $0$-APE-$K$ for each arm. We can observe that the major difference in sample complexity is due to 2 being over-sampled by \algauername. 
\begin{figure}[ht]
     \centering
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
    \includegraphics[width=\textwidth]{data/E/instance-new.pdf}
         \caption{Instance}
         \label{fig:config-avantage-APE}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
    \includegraphics[width=\textwidth]{data/E/new-instance-ape-k-results.pdf}
         \caption{Sample complexity}
         \label{fig:appx-new-instance-ape-k-sc}
     \end{subfigure}
        \caption{For this instance (left) $\cS^\star = \{0,2, 3\}$. The figure at right is the average sample complexity on the across the trials on the same instance.}
        \label{fig:appx-new-instance-ape-k-results}
\end{figure} 
\begin{table}[htb]
    \centering
    \begin{tabular}{c|c}
    \hline 
      Arm    &  Average ratio of pulls\\\hline 
      0   & 3.08 \\
      1 & 1.36 \\
      2 & 5.68 \\
      3 & 1.28 \\
      4 & 1.40 \\
    \end{tabular}
    \caption{Average number of pulls taken  by \algauername divided by the average number of pulls taken by $0$-APE-$K$ for each arm.}
    \label{tab:average-pull-ratio}
\end{table}

By increasing the number of arms and the dimension we can generate instances similar to \autoref{fig:config-avantage-APE} when the gap between our algorithm and \algauername is even larger. For a specific instance where $K=12$, $D=10$ and there are 11 optimal arms. On this instance, we can see that our algorithm uses 3 times less samples than \algauername. 
\begin{figure}
    \centering
    \includegraphics[width=0.6\linewidth]{data/E/new-instance-ape-k-results2.pdf}
    \caption{Average sample complexity on a specific instance with $K=12, D=10$ and 11 optimal arms}
    \label{fig:appx-new-instance-higher-dim}
\end{figure}

% \begin{minipage}[b]{0.45\linewidth}
% \centering
% \begin{tabular}{c|cccccccccc}
% Arm & \multicolumn{10}{c}{$\vmu$}\\\hline 
% 0 & 0.80 & 0.09 & 0.21 & 0.71 & 0.86 & 0.41 & 0.85 & 0.27 & 0.53 & 0.46\\
%   1& 0.68 & 0.41 & 0.51 & 0.96 & 0.95 & 0.05 & 0.48 & 0.87 & 0.84 & 0.67\\
%   2&0.74 & 0.94 & 0.41 & 0.04 & 0.20 & 0.49 & 0.48 & 0.93 & 0.38 & 0.73\\
%   3&0.63 & 0.39 & 0.54 & 0.96 & 0.18 & 0.69 & 0.41 & 0.62 & 0.41 & 0.53\\
%   4&0.96 & 0.96 & 0.17 & 0.36 & 0.87 & 0.53 & 0.12 & 0.84 & 0.55 & 0.97\\
%   5&0.74 & 0.05 & 0.30 & 0.62 & 0.28 & 0.45 & 0.99 & 0.44 & 0.55 & 0.42\\
%   6&0.33 & 0.27 & 0.35 & 0.05 & 0.09 & 0.94 & 0.64 & 0.93 & 0.20 & 0.71\\
%   7&0.04 & 0.08 & 0.05 & 0.02 & 0.17 & 0.07 & 0.09 & 0.11 & 0.17 & 0.33\\
%   8&0.56 & 0.83 & 0.64 & 0.74 & 0.70 & 0.79 & 0.47 & 0.55 & 0.21 & 0.67\\
%   9&0.19 & 0.34 & 0.67 & 0.13 & 0.59 & 0.08 & 0.34 & 0.78 & 0.73 & 0.19\\
%   10&0.95 & 0.50 & 0.06 & 0.57 & 0.30 & 0.60 & 0.69 & 0.56 & 0.17 & 0.38\\
%   11&0.56 & 0.57 & 0.98 & 0.08 & 0.06 & 0.22 & 0.62 & 0.91 & 0.25 & 0.06\\\hline 
%   \end{tabular}
%     \caption{Caption}
%     \label{tab:my_label}
% \end{minipage} \hfill
% \begin{minipage}[c]{0.45\linewidth}
% [...]
% \end{minipage}
% Therefore, by taking an instance where they're many optimal arms which all dominates the same sub-optimal arm, we expect from our sampling rule that when this sub-optimal arm is sampled as $b_t$ to sample $c_t$ the optimal arm which is dominates $b_t$ with the largest gap. 
% % figure 
% array([[0.37823179, 0.96332576],
%        [0.52483929, 0.25693304],
%        [0.85350985, 0.26768743],
%        [0.59589704, 0.63565148],
%        [0.34267242, 0.56729502]])

% The means of the arms are given in the table below \autoref{tab:arith_mean}. We have  $\cS^\star(\mathbf{A}) = \{0, 2, 3\}$ and $\cS^\star(\mathbf{A}) = \{\}$. We set $\eps_1=0$ for both algorithms and we use the stopping time $\tau_\delta^{\eps_1}$ for \algname.  
%% minipage 
\subsubsection{$\eps_2$-relaxation}
%\paragraph{Experiments:}
We assess the empirical performance performance of \algname associate to $\tau_{\eps_1, \eps_2}$ for identifying an $(\eps_1, \eps_2)-$cover.  We set $\eps_1=0, \delta=0.01$ and we test different values of $\eps_2 \in \{0, 0.05, 0.1, 0.2, 0.25\}$. We average the results over 5000 independent trials with different seeds on the same instance. We use multi-variate Bernoulli with independent marginals (not required). The instance of \autoref{fig:config_eps_2} is a toy example where $(\eps_1, \eps_2)-$covering can be meaningful and reduce the sample complexity. The 3 {Pareto optimal} vectors are chosen by hand and the last 2 vectors are randomly uniformly generated. 
% figure a cote avec les boxplot fonction de eps_2
%TODO remplacer la figure 
\begin{figure}[ht]
     \centering
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
    \includegraphics[width=\textwidth]{data/C/instance.pdf}
         \caption{Instance}
         \label{fig:config_eps_2}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
    \includegraphics[width=\textwidth]{data/C/result.png}
         \caption{Sample complexity}
         \label{fig:appx-C-results-result}
     \end{subfigure}
        \caption{For this instance (left) $\cS^\star = \{0,1,2\}$. The difference in on \texttt{x} and \texttt{y} axis is $0.1$ between arm 0 and 1 and $0.05$ between arm 1 and 2. The figure at right is the average sample complexity on the across the trials on the same instance.}
        \label{fig:appx-C-results}
\end{figure}
We can observe on \autoref{fig:appx-C-results-result} that the sample complexity decreases as $\eps_2$ increases. This is further confirmed in \autoref{fig:appx-C-results_eps_2} which shows the empirical sample complexity and the average size of the recommended cover versus $\eps_2$ for 50 equally-spaced values of $\eps_2$ between $0$ and $1/2$.  The drops observed in \autoref{fig:appx-C-sample_complexity_vs_eps_2} correspond to the values of $\eps_2$ for which \algname chooses to remove an \emph{optimal} arm from the cover to save some samples (\autoref{fig:appx-C-average_card_O}). A major decrease in the sample complexity corresponds more or less to an arm being removed from the recommended set. 
% \autoref{fig:appx-C-results-result}  and \autoref{fig:appx-C-sample_complexity_vs_eps_2} which show empirically the impact of $\eps_2$ on the sample complexity and the number of arms in the recommended cover. 
\begin{figure}[htb]
     \centering
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
    \includegraphics[width=\textwidth]{data/C/result_card_vs_eps.png}
         \caption{Average $\lvert\cO({\tau_{\eps_1, \eps_2}})\lvert$  vs $\eps_2$}
         \label{fig:appx-C-average_card_O}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
    \includegraphics[width=\textwidth]{data/C/result_tau_vs_eps.png}
         \caption{Sample complexity vs $\eps_2$}
         \label{fig:appx-C-sample_complexity_vs_eps_2}
     \end{subfigure}
        \caption{On the left is the average length of $\cO_{\tau_\delta}$ (over the different seeds) versus $\eps_2$ and on the right is the empirical sample complexity (averaged over the runs) versus $\eps_2$. We check that the algorithm is correct. The y-axis represents the number of times the arm has been recommended across the runs with different seeds.}
        \label{fig:appx-C-results_eps_2}
\end{figure}
The plateau in the sample complexity for large values of $\eps_2$ ($>0.3$) is explained by the fact the algorithm needs to identify at least one \emph{optimal} arm (which is reflected in the size of the returned set \autoref{fig:appx-C-average_card_O}).
Indeed, for $\eps_1=0$ fixed, an algorithm for $(\eps_1, \eps_2)-$cover still needs to assert that the arms in the recommended set are truly optimal which will require some samples even when $\eps_2$ is very large. 
\subsubsection{Comparing $\eps_1$-APE-$k$ to an heuristic}
In this section, we compare $\eps_1$-APE-$k$ to the heuristic version of \algauername which stops as soon as at $k$ optimal arms have been identified. The pseudo-code of the algorithm is given in \autoref{alg:heuristic-auer}. As shown in \cite{auer_pareto_2016}, arms in $P_1(t)$ are already identified as optimal but when the goal is to identify the Pareto set, some of them (namely $P_1(t)\backslash P_2(t)$) need to be sampled again until all the arms they potentially dominate are removed from $A(t)$ and then those arms will belong to $P_2(t)$ and will be removed from the active set. However, for the $k$-relaxation, identifying $k$ optimal arms is enough so the algorithm can stop as soon as $\lvert P(t-1) \cup P_1(t)\lvert \geq k$. It this never occur, then the algorithm will follow the initial stopping condition, that is when $A(t) = \emptyset$. 

\begin{algorithm}[htb]
\caption{Heuristic \algauername for the $k$-relaxation}\label{alg:heuristic-auer}
\KwData{parameter $\eps_1\geq 0, k\leq K$}
\Input{$A(0) = \bA$, $t \gets 1$, $P(0) = P_1(0) = P_2(0) = \emptyset$ } 
 \For{$t=1,2,\dots$}{
 \Sample each arm in $A(t-1)$ once \;
 $A(t) \gets  \{i \in A(t-1): \forall \; j\in A(t-1), \mh(i,j,t)\leq \beta_{i,j}(t)\} $\; 
$P_1(t) \gets  \{ i \in A_1(t): \forall\; j\in A_1(t)\setminus \{i\}, \tilde\Mh_{\eps_1}(i,j,t)\geq  \beta_{i,j}(t) \}$\;
$P_2(t) \gets \{ j \in P_1(t): \nexists \;i \in A_1(t)\setminus P_1(t) \tm{ s.t } \tilde \Mh_{\eps_1}(i,j,t)\leq \beta_{i,j}(t)\}$\;
$A(t)\gets A_1(t) \setminus P_2(t)$ and $P(t) \gets  P(t-1) \cup P_2(t)$\;
\If{$ A(t) = \emptyset$}{
\textbf{break} and output $P(t)$\;
}
\If{$\lvert P(t-1) \cup P_1(t)\lvert \geq k$}{
\textbf{break} and output $P(t-1) \cup P_1(t)$\;
}
  $t \gets t + 1$\;
 }
\end{algorithm}
We set $\delta = 0.1$ and $\eps_1 = 0.005$ and run both algorithms on 2000 random Bernoulli instances with $K=5, D=2$. 
\autoref{fig:appx-comp-ape-heuristic} shows the performance of the average sample complexity of the algorithms for each value of $k \in \{1, \dots, 5\}$

\begin{figure}
    \centering
    \includegraphics{data/A/comp-ape-heuristic.pdf}
    \caption{Caption}
    \label{fig:appx-comp-ape-heuristic}
\end{figure}
